Leveraging Transformer-based Language Models to Automate Requirements Satisfaction Assessment

Requirements Satisfaction Assessment (RSA) evaluates whether the set of design elements linked to a single requirement provide sufficient coverage of that requirement -- typically meaning that all concepts in the requirement are addressed by at least one of the design elements. RSA is an important software engineering activity for systems with any form of hierarchical decomposition -- especially safety or mission critical ones. In previous studies, researchers used basic Information Retrieval (IR) models to decompose requirements and design elements into chunks, and then evaluated the extent to which chunks of design elements covered all chunks in the requirement. However, results had low accuracy because many critical concepts that extend across the entirety of the sentence were not well represented when the sentence was parsed into independent chunks. In this paper we leverage recent advances in natural language processing to deliver significantly more accurate results. We propose two major architectures: Satisfaction BERT (Sat-BERT), and Dual-Satisfaction BERT (DSat-BERT), along with their multitask learning variants to improve satisfaction assessments. We perform RSA on five different datasets and compare results from our variants against the chunk-based legacy approach. All BERT-based models significantly outperformed the legacy baseline, and Sat-BERT delivered the best results returning an average improvement of 124.75% in Mean Average Precision.

==> tables/BaselineC2.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table*}[t!]
\centering
\addtolength{\tabcolsep}{-3pt}
\caption{Performance of traditional approaches on C2 challenge (Coverage Score and Coverage Rate reported the same results). We report the MAPs and F2s based on the number of design elements that a requirement possess. The final column reports the average scores, which is used as our legacy baseline.}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\begin{tabular}{|c|c|cc|cc|cc|cc|cc|cc|cc|} 
\hline
\multirow{2}{*}{\bf Challenge} & \multirow{2}{*}{Datasets} & \multicolumn{2}{c|}{2} & \multicolumn{2}{c|}{3} & \multicolumn{2}{c|}{4 $\lozenge$} & \multicolumn{2}{c|}{5} & \multicolumn{2}{c|}{6} & \multicolumn{2}{c|}{7} & \multicolumn{2}{c|}{9} \\ 

 & & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP \\
\hline
\multirow{5}{*}{C2} & CM1 & 0.835 & 0.556 & 0.714 & 0.350 & 0.409 & 0.137 & 0.261 & 0.069 & 0.141 & 0.033 & - & - & - & - \\ 

 & CCHIT & 0.821 & 0.483 & 0.550 & 0.207 & 0.553 & 0.213 & 0.225 & 0.058 & 0.128 & 0.028 & 0.122 & 0.033 & 0.014 &0.003\\ 

 & Dronology & 0.790 & 0.467 & 0.507 & 0.174 & 0.327 & 0.090 & 0.191 & 0.046 & - & - & - & - & 0.010 & 0.002 \\ 

 & PTC & 0.841 & 0.571 & 0.599 & 0.245 & 0.562 & 0.237 & 0.293 & 0.077 & 0.158 & 0.038 & - & - & - & - \\ 

 & PTC-1 & 0.868 & 0.656 & 0.658 & 0.317 & 0.583 & 0.250 & - & - & - & - & - & - & - & - \\
\hline
\end{tabular}
\end{table*}

% 0.345	0.147
% 0.365	0.156
% 0.491	0.234
% 0.703	0.407

==> tables/Baselines.tex <==



\begin{table}
\centering
\addtolength{\tabcolsep}{-4pt}
\caption{Performance of traditional approaches on challenges C1, and C3 against two datasets i.e. CM-1 and Dronology. We use F2 and MAP as our evaluation metrics. However, we do not report the F-2 score for the C3 challenge as it is a multi-class classification problem. In addition, the final column of the table reports the maximum F2 and MAP from two approaches, which we use as our Legacy Baseline.}
\scalebox{0.9}{
\begin{tabular}{c|c|c|cc|cc|cc} 
\hline
\multicolumn{1}{c|}{}  &\multicolumn{1}{c|}{Datasets}  & \multicolumn{1}{c|}{Samples(k)} 
&\multicolumn{2}{c|}{Coverage Rate} &\multicolumn{2}{c|}{Coverage Score}  & \multicolumn{2}{c}{MAX (L-Baseline)}  \\ 

\multirow{6}{*}{C1}  & & & F2  & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2}  & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2}  & \multicolumn{1}{c}{MAP} \\ 
\hline

  & \multirow{3}{*}{CM1}  & 100  & 0.111 & 0.132  & 0.115 & 0.199  & 0.115 & 0.199  \\ 

  &  & 300  & 0.051 & 0.105  & 0.058 & 0.167  & 0.058 & 0.167  \\ 

  &  & 500  & 0.041 & 0.104  & 0.046 & 0.166  & 0.046 & 0.166  \\ 

\cline{2-9}
  & \multirow{3}{*}{Dronology} & 100  & 0.106 & 0.293  & 0.114 & 0.285  & 0.114 & 0.293  \\ 

  &  & 300  & 0.041 & 0.234  & 0.042 & 0.224  & 0.042 & 0.234  \\ 

  &  & 500  & 0.026 & 0.233  & 0.028 & 0.223  & 0.028 & 0.233  \\ 
\hline

\multirow{7}{*}{C3} & \multirow{3}{*}{CM1}  & 100  & -  & 0.140  & -  & 0.200  & -  & 0.200  \\ 

  &  & 300  & -  & 0.105  & -  & 0.167  & -  & 0.167  \\ 

  &  & 500  & -  & 0.104  & -  & 0.166  & -  & 0.166  \\ 
\cline{2-9}

  & \multirow{3}{*}{Dronology} & 100  & -  & 0.270  & -  & 0.267  & -  & 0.270  \\ 

  & \multicolumn{1}{c|}{}  & 300  & -  & 0.254  & -  & 0.244  & -  & 0.254  \\ 

  & \multicolumn{1}{c|}{}  & 500  & -  & 0.233  & -  & 0.223  & -  & 0.233  \\
\hline
\end{tabular}
}
L-Baseline = Legacy Baseline
\end{table}




% % \usepackage{multirow}
% % \usepackage{colortbl}

% \begin{table}[!tb]
% \centering
% \caption{L2PLUS-Baseline -- two approaches -- Coverage Rate and Coverage Score}
% \scalebox{0.7}{
% \begin{tabular}{c|c|cc|cc|cc}\toprule \hline
% L2-PLUS  &Samples  & \multicolumn{2}{c|}{Coverage Rate} & \multicolumn{2}{c|}{Coverage Score}  &\multicolumn{2}{c}{MAX (L-Baseline)} \\ 
% &  & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP}  & \multicolumn{1}{c}{F2}  & \multicolumn{1}{c}{MAP} \\ 
% \hline

% \multirow{3}{*}{CM1}  & 100  & -  & 0.140  & -  & 0.200  & -  & 0.200  \\ 

%  & 300  & -  & 0.105  & -  & 0.167  & -  & 0.167  \\ 

%  & 500  & -  & 0.104  & -  & 0.166  & -  & 0.166  \\ 
% \hline

% \multirow{3}{*}{Dronology} & 100  & -  & 0.270  & -  & 0.267  & -  & 0.270  \\ 

%  & 300  & -  & 0.254  & -  & 0.244  & -  & 0.254  \\ 

%  & 500  & -  & 0.233  & -  & 0.223  & -  & 0.233  \\

% \hline
% \end{tabular}}
% \end{table}


% \usepackage{multirow}
% \usepackage{colortbl}

==> tables/BaselinesC1C3.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}
\begin{table*}
\centering
\caption{Performance of traditional approaches on challenges C1, and C3. The max column reports the maximum score from the two approaches, whereas the final column reports the average score across three samples from Max, which is used as our legacy baseline.}
\addtolength{\tabcolsep}{-3.5pt}
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|c|c|c|r|c|r|c|r|c|r|} 
\hline
\multicolumn{2}{|c|}{} & \multicolumn{6}{c|}{Coverage Rate} & \multicolumn{6}{c|}{Coverage Score} & \multicolumn{6}{c|}{Max} & \multicolumn{2}{c|}{} \\ 

% \multicolumn{1}{|l|}{} & & \multicolumn{6}{c|}{Coverage Rate} & \multicolumn{6}{c|}{Coverage Score} & \multicolumn{6}{c|}{Max (Legacy -Baseline)} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ 
\cline{3-20}

\multicolumn{2}{|c|}{{\bf Challenges}} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300} & \multicolumn{2}{c|}{500} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300} & \multicolumn{2}{c|}{500} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300} & \multicolumn{2}{c|}{500} & \multicolumn{2}{c|}{Avg Results $\lozenge$} \\ 

\multicolumn{2}{|c|}{}& \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP}\\ 

%  & \multicolumn{1}{c|}{} & F2 & MAP & F2 & MAP & F2 & MAP & F2 & MAP & F2 & MAP & F2 & MAP & F2 & \multicolumn{1}{c|}{MAP} & F2 & \multicolumn{1}{c|}{MAP} & F2 & \multicolumn{1}{c|}{MAP} & F2 & \multicolumn{1}{c|}{MAP} \\ 
\hline
\multirow{5}{*}{C1} & CM1 & 0.111 & 0.132 & 0.051 & 0.105 & 0.041 & 0.104 & 0.115 & 0.199 & 0.058 & 0.167 & 0.046 & 0.166 & \multicolumn{1}{r|}{0.115} & 0.199 & \multicolumn{1}{r|}{0.058} & 0.167 & \multicolumn{1}{r|}{0.046} & 0.166 & \multicolumn{1}{r|}{0.073} & 0.177 \\ 

 & CCHIT & 0.062 & 0.016 & 0.023 & 0.008 & 0.016 & 0.007 & 0.064 & 0.016 & 0.025 & 0.008 & 0.019 & 0.007 & \multicolumn{1}{r|}{0.064} & 0.016 & \multicolumn{1}{r|}{0.025} & 0.008 & \multicolumn{1}{r|}{0.019} & 0.007 & \multicolumn{1}{r|}{0.036} & 0.010 \\ 

 & Dronology & 0.106 & 0.293 & 0.041 & 0.234 & 0.026 & 0.233 & 0.114 & 0.285 & 0.042 & 0.224 & 0.028 & 0.223 & \multicolumn{1}{r|}{0.114} & 0.293 & \multicolumn{1}{r|}{0.042} & 0.234 & \multicolumn{1}{r|}{0.028} & 0.233 & \multicolumn{1}{r|}{0.061} & 0.253 \\ 

 & PTC & 0.145 & 0.264 & 0.065 & 0.173 & 0.045 & 0.170 & 0.158 & 0.310 & 0.069 & 0.214 & 0.047 & 0.210 & \multicolumn{1}{r|}{0.158} & 0.310 & \multicolumn{1}{r|}{0.069} & 0.214 & \multicolumn{1}{r|}{0.047} & 0.210 & \multicolumn{1}{r|}{0.091} & 0.245 \\ 

 & PTC-1 & 0.158 & 0.210 & 0.105 & 0.162 & 0.097 & 0.162 & 0.164 & 0.254 & 0.107 & 0.205 & 0.096 & 0.205 & \multicolumn{1}{r|}{0.164} & 0.254 & \multicolumn{1}{r|}{0.107} & 0.205 & \multicolumn{1}{r|}{0.097} & 0.205 & \multicolumn{1}{r|}{0.123} & 0.221 \\ 

\hline
\multirow{4}{*}{C3} & CM1 & - & 0.140 & - & 0.105 & - & 0.104 & - & 0.200 & - & 0.167 & - & 0.166 & - & 0.200 & - & 0.167 & - & 0.166 & - & 0.178 \\ 

 & CCHIT & - & 0.016 & - & 0.008 & - & 0.007 & - & 0.016 & - & 0.008 & - & 0.007 & - & 0.016 & - & 0.008 & - & 0.007 & - & 0.010 \\ 

 & Dronology & - & 0.270 & - & 0.254 & - & 0.233 & - & 0.267 & - & 0.244 & - & 0.223 & - & 0.270 & - & 0.254 & - & 0.233 & - & 0.252 \\ 

 & PTC & - & 0.257 & - & 0.174 & - & 0.170 & - & 0.314 & - & 0.215 & - & 0.210 & - & 0.314 & - & 0.215 & - & 0.210 & - & 0.246 \\ 

\multicolumn{1}{|l|}{} & PTC-1 & - & 0.205 & - & 0.162 & - & 0.162 & - & 0.205 & - & 0.162 & - & 0.162 & - & 0.205 & - & 0.162 & - & 0.162 & - & 0.177 \\
\hline
\end{tabular}
\end{table*}


% \begin{table*}[t!]
% \centering
% \caption{Performance of traditional approaches on challenges C1, and C3. The final column of the table reports the maximum F2 and MAP from the two approaches for each sample size, which we use as our Legacy Baseline.}
% %\scalebox{0.84}{
% % \begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|c|c|c|r|c|r|c|r|}
% \addtolength{\tabcolsep}{-2.3pt}
% \begin{tabular}{|c|l|cc|cc|cc|cc|cc|cc|cc|cc|cc|} 
% \hline

% \multicolumn{2}{|c|}{} & \multicolumn{6}{c|}{Coverage Rate} & \multicolumn{6}{c|}{Coverage Score} & \multicolumn{6}{c|}{Max (Legacy -Baseline $\lozenge$)} \\ 

% \cline{3-20}
%  \multicolumn{2}{|c|}{{\bf Challenges}} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300} & \multicolumn{2}{c|}{500} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300} & \multicolumn{2}{c|}{500} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300} & \multicolumn{2}{c|}{500} \\ 

% \multicolumn{2}{|c|}{}& \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} \\ 
 
% \hline

% \multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering C1}}} 
%  & CM1 & 0.111 & 0.132 & 0.051 & 0.105 & 0.041 & 0.104 & 0.115 & 0.199 & 0.058 & 0.167 & 0.046 & 0.166 & 0.115 & 0.199 & 0.058 & 0.167 & 0.046 & 0.166 \\ 

%  & CCHIT & 0.062 & 0.016 & 0.023 & 0.008 & 0.016 & 0.007 & 0.064 & 0.016 & 0.025 & 0.008 & 0.019 & 0.007 & 0.064 & 0.016 & 0.025 & 0.008 & 0.019 & 0.007 \\ 

%  & Dronology & 0.106 & 0.293 & 0.041 & 0.234 & 0.026 & 0.233 & 0.114 & 0.285 & 0.042 & 0.224 & 0.028 & 0.223 & 0.114 & 0.293 & 0.042 & 0.234 & 0.028 & 0.233 \\ 

%  & PTC & 0.145 & 0.264 & 0.065 & 0.173 & 0.045 & 0.170 & 0.158 & 0.310 & 0.069 & 0.214 & 0.047 & 0.210 & 0.158 & 0.310 & 0.069 & 0.214 & 0.047 & 0.210 \\ 
 
%  &PTC-1 & 0.158 & 0.210 & 0.105 & 0.162 & 0.097 & 0.162 & 0.164 & 0.254  & 0.107 & 0.205    & 0.096 & 0.205 & 0.164 & 0.254                 & 0.107 & 0.205                 & 0.097 & 0.205                  \\ 
 
% \hline
% \multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering C3}}} 
%  & CM1 & - & 0.140 & - & 0.105 & - & 0.104 & - & 0.200 & - & 0.167 & - & 0.166 & - & 0.200 & - & 0.167 & - & 0.166 \\ 

%  & CCHIT & - & 0.016 & - & 0.008 & - & 0.007 & - & 0.016 & - & 0.008 & - & 0.007 & - & 0.016 & - & 0.008 & - & 0.007 \\ 

%  & Dronology & - & 0.270 & - & 0.254 & - & 0.233 & - & 0.267 & - & 0.244 & - & 0.223 & - & 0.270 & - & 0.254 & - & 0.233 \\ 

%  & PTC & - & 0.257 & - & 0.174 & - & 0.170 & - & 0.314 & - & 0.215 & - & 0.210 & - & 0.314 & - & 0.215 & - & 0.210 \\
 
%  &PTC-1  & -     & 0.205 & -& 0.162 & - & 0.162 & - & 0.205 & -& 0.162  & - & 0.162 & -  & 0.205 & -  & 0.162 & - & 0.162                  \\
 
% \hline
% \end{tabular}
% %}
% \end{table*}


% \usepackage{multirow}
% \usepackage{colortbl}




==> tables/BaselinesModified.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multicolumn{1}{|l|}{} & & \multicolumn{6}{c|}{Coverage Rate} & \multicolumn{6}{c|}{Coverage Score} \\ 
\cline{3-14}
\multirow{2}{*}{Challenges} & \multicolumn{1}{c|}{\multirow{2}{*}{Datasets}} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300} & \multicolumn{2}{c|}{500} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300} & \multicolumn{2}{c|}{500} \\ 

 & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP \\ 
\hline
\multirow{4}{*}{C1} & CM1 & 0.111 & 0.132 & 0.051 & 0.105 & 0.041 & 0.104 & 0.115 & 0.199 & 0.058 & 0.167 & 0.046 & 0.166 \\ 

 & CCHIT & 0.062 & 0.016 & 0.023 & 0.008 & 0.016 & 0.007 & 0.064 & 0.016 & 0.025 & 0.008 & 0.019 & 0.007 \\ 

 & Dronology & 0.106 & 0.293 & 0.041 & 0.234 & 0.026 & 0.233 & 0.114 & 0.285 & 0.042 & 0.224 & 0.028 & 0.223 \\ 

 & PTC & 0.145 & 0.264 & 0.065 & 0.173 & 0.045 & 0.170 & 0.158 & 0.310 & 0.069 & 0.214 & 0.047 & 0.210 \\ 
\hline

\multirow{4}{*}{C3} & CM1 & - & 0.140 & - & 0.105 & - & 0.104 & - & 0.200 & - & 0.167 & - & 0.166 \\ 

 & CCHIT & - & 0.016 & - & 0.008 & - & 0.007 & - & 0.016 & - & 0.008 & - & 0.007 \\ 

 & Dronology & - & 0.270 & - & 0.254 & - & 0.233 & - & 0.267 & - & 0.244 & - & 0.223 \\ 

 & PTC & - & 0.257 & - & 0.174 & - & 0.170 & - & 0.314 & - & 0.215 & - & 0.210 \\
\hline
\end{tabular}
\end{table*}

==> tables/C1-single-avg.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}

% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table*}[t!]
\addtolength{\tabcolsep}{-0.5pt}
\centering
\caption{Performance of various language models leveraging single and dual BERT based model architecture on C1 challenge. $\lozenge$ is a baseline for bert\_sat, whereas $\blacklozenge$ is a baseline for all other models.}
\begin{tabular}{|c|l|r|r|r|r|r|r|r|r|r|r|r|r|} 
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Arch}} & \multirow{2}{*}{\textbf{Challenge C1}} & \multicolumn{2}{c|}{CM1} & \multicolumn{2}{c|}{CCHIT} & \multicolumn{2}{c|}{Dronology} & \multicolumn{2}{c|}{PTC} & \multicolumn{2}{c|}{PTC-1} & \multicolumn{2}{c|}{Average Improve} \\ 

\multicolumn{1}{|l|}{} & & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} \\ 

\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering Sat-BERT MSat-BERT}}}
& legacy $\lozenge$ & 0.073 & 0.177 & 0.036 & 0.010 & 0.061 & 0.253 & 0.091 & 0.245 & 0.123 & 0.221 & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ 

 & bert\_sat $\blacklozenge$ & 0.163 & 0.206 & 0.175 & 0.105 & 0.423 & 0.535 & 0.473 & 0.534 & 0.484 & 0.579 & 362.34\% & 264.78\% \\ 

 & bert\_mul & 0.217 & 0.272 & 0.233 & 0.179 & 0.442 & 0.566 & 0.462 & 0.557 & 0.493 & 0.564 & 13.90\% & 22.13\% \\ 

 & scibert\_sat & 0.255 & 0.263 & 0.262 & \textbf{0.287} & 0.473 & 0.612 & \textbf{0.509} & \textbf{0.591} &\textbf{ 0.524} & \textbf{0.599} & 26.68\% & \textbf{45.94\%} \\ 

 & scibert\_mul & 0.274 & 0.288 & \textbf{0.270} & 0.224 & 0.478 & 0.636 & 0.499 & 0.573 & 0.481 & 0.542 & \textbf{28.02\%} & 34.72\% \\ 

 & sebert\_sat & 0.252 & 0.278 & 0.161 & 0.101 & \textbf{0.541} & \textbf{0.672} & 0.456 & 0.560 & 0.419 & 0.506 & 11.41\% & 9.77\% \\ 

 & sebert\_mul &\textbf{ 0.298} & \textbf{0.359} & 0.172 & 0.109 & 0.520 & 0.626 & 0.470 & 0.555 & 0.402 & 0.469 & 17.30\% & 15.98\% \\ 

\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering DSat-BERT DMSat-BERT}}}
& bert\_sat & 0.185 & 0.202 & 0.221 & 0.184 & 0.450 & 0.587 & 0.433 & 0.534 & 0.456 & 0.570 & 6.29\% & 16.34\% \\ 

 & bert\_mul & 0.221 & 0.268 & 0.222 & 0.151 & 0.450 & 0.550 & 0.468 & 0.551 & 0.475 & 0.563 & 13.08\% & 15.48\% \\ 

 & scibert\_sat & 0.249 & 0.279 & 0.225 & \textbf{0.271} & 0.440 & 0.530 & 0.487 & 0.552 & \textbf{0.510} & \textbf{0.585} & 18.62\% & \textbf{39.45\%} \\ 

 & scibert\_mul & 0.266 & 0.308 & \textbf{0.243} & 0.218 & 0.493 & 0.604 & \textbf{0.491} & \textbf{0.571} & 0.509 & 0.577 & \textbf{25.38\%} & 35.41\% \\ 

 & sebert\_sat & 0.240 & 0.266 & 0.184 & 0.122 & 0.510 & 0.596 & 0.400 & 0.526 & 0.369 & 0.452 & 6.62\% & 6.82\% \\ 

 & sebert\_mul &\textbf{ 0.289} & \textbf{0.313} & 0.210 & 0.166 & \textbf{0.543} & \textbf{0.607} & 0.420 & 0.513 & 0.397 & 0.453 & 19.31\% & 19.48\% \\
\hline
\end{tabular}
\end{table*}


% \begin{table*}[t!]
% \centering
% \caption{Performance of various language models leveraging single BERT based model architecture on C1 challenge. Average improvement results (right hand side) represent comparisons against the baselines.}
% \begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|} 
% \hline
% \multirow{2}{*}{\textbf{Challenge C1}} & \multicolumn{2}{c|}{CM1} & \multicolumn{2}{c|}{CCHIT} & \multicolumn{2}{c|}{Dronology} & \multicolumn{2}{c|}{PTC} & \multicolumn{2}{c|}{PTC-1} & \multicolumn{2}{c|}{Average Improve} \\ 

%  & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} \\ 
% \hline
% legacy $\lozenge$ & 0.073 & 0.177 & 0.036 & 0.010 & 0.061 & 0.253 & 0.091 & 0.245 & 0.123 & 0.221 & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} \\ 

% bert\_sat $\blacklozenge$ & 0.163 & 0.206 & 0.175 & 0.105 & 0.423 & 0.535 & 0.473 & 0.534 & 0.484 & 0.579 & 362.34\% & 264.78\% \\ 

% bert\_mul & 0.217 & 0.272 & 0.233 & 0.179 & 0.442 & 0.566 & 0.462 & 0.557 & 0.493 & 0.564 & 13.90\% & 22.13\% \\ 

% scibert\_sat & 0.255 & 0.263 & 0.262 & 0.287 & 0.473 & 0.612 & 0.509 & 0.591 & 0.524 & 0.599 &\textbf{ 21.87}\% & \textbf{28.71}\% \\ 

% scibert\_mul & 0.274 & 0.288 & 0.270 & 0.224 & 0.478 & 0.636 & 0.499 & 0.573 & 0.481 & 0.542 & 20.36\% & 14.79\% \\ 

% sebert\_sat & 0.252 & 0.278 & 0.161 & 0.101 & 0.541 & 0.672 & 0.456 & 0.560 & 0.419 & 0.506 & 4.73\% & 2.47\% \\ 

% sebert\_mul & 0.298 & 0.359 & 0.172 & 0.109 & 0.520 & 0.626 & 0.470 & 0.555 & 0.402 & 0.469 & 8.04\% & 8.64\% \\
% \hline
% \end{tabular}
% % $\blacklozenge$ = Baseline for the BERT-based models, Variants of single task variants are suffixed as \_sat, whereas the multitask variants are suffixed as \_mul.\\
% % $\lozenge$=Legacy results using VSM without use of BERT models.
% \end{table*}

==> tables/C2-single-avg.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table*}[t!]
\centering
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Arch}} & \multirow{2}{*}{\textbf{Challenge C2}} & \multicolumn{2}{c|}{CM1} & \multicolumn{2}{c|}{CCHIT} & \multicolumn{2}{c|}{Dronology} & \multicolumn{2}{c|}{PTC} & \multicolumn{2}{c|}{PTC-1} & \multicolumn{2}{c|}{Average Improve} \\ 

\multicolumn{1}{|l|}{} & & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} \\ 
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering Sat-BERT MSat-BERT}}}
& legacy & 0.472 & 0.229 & 0.345 & 0.147 & 0.365 & 0.156 & 0.491 & 0.234 & 0.703 & 0.407 & - & - \\ 

 & bert\_sat & 0.830 & 0.688 & 0.824 & 0.690 & 0.834 & 0.765 & 0.766 & 0.590 & 0.847 & 0.693 & 84.02\% & 237.11\% \\ 

 & bert\_mul & 0.865 & 0.731 & 0.724 & 0.593 & 0.792 & 0.736 & 0.854 & 0.755 & \textbf{0.955} & \textbf{0.896} & 2.26\% & 9.10\% \\ 

 & scibert\_sat & 0.904 & 0.813 & 0.898 & 0.804 & \textbf{0.931} & \textbf{0.855} & 0.832 & 0.719 & 0.900 & 0.817 & \textbf{8.88}\% & 17.24\% \\ 

 & scibert\_mul & \textbf{0.955} & \textbf{0.889} & \textbf{0.909} & \textbf{0.833} & 0.832 & 0.756 & 0.873 & 0.777 & 0.887 & 0.744 & 8.76\% & \textbf{17.58}\% \\ 

 & sebert\_sat & 0.940 & 0.877 & 0.798 & 0.697 & 0.842 & 0.760 & \textbf{0.876} &\textbf{0.782} & 0.884 & 0.772 & 5.96\% & 14.35\% \\ 

 & sebert\_mul & 0.873 & 0.746 & 0.858 & 0.767 & 0.819 & 0.760 & 0.835 & 0.676 & 0.860 & 0.717 & 3.61\% & 7.37\% \\ 

\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering DSat-BERT DMSat-BERT}}} & bert\_sat & 0.801 & 0.665 & 0.889 & 0.748 & 0.735 & 0.619 & 0.625 & 0.457 & 0.899 & 0.785 & -3.95\% & -4.63\% \\ 

 & bert\_mul & 0.826 & 0.692 & 0.769 & 0.663 & 0.730 & 0.605 & 0.726 & 0.576 & 0.926 & 0.828 & -3.08\% & -1.43\% \\ 

 & scibert\_sat & 0.884 & 0.799 & 0.839 & 0.721 & 0.798 & 0.683 & 0.774 & 0.641 & 0.948 & 0.856 & 3.39\% & 8.38\% \\ 

 & scibert\_mul & 0.841 & 0.717 & 0.942 & 0.893 & 0.848 & 0.757 & 0.752 & 0.595 & 0.956 & 0.906 & 5.67\% & 12.84\% \\ 

 & sebert\_sat & 0.874 & 0.755 & 0.897 & 0.840 & 0.790 & 0.665 & 0.707 & 0.536 & 0.968 & 0.917 & 3.10\% & 8.30\% \\ 

 & sebert\_mul & 0.818 & 0.705 & 0.875 & 0.825 & 0.804 & 0.724 & 0.717 & 0.535 & 0.940 & 0.892 & 1.16\% & 7.23\% \\
\hline
\end{tabular}
\end{table*}

==> tables/C3-single-avg.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}

% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table*}[t!]
\addtolength{\tabcolsep}{-0.5pt}
\centering
\caption{Performance of various language models leveraging single and dual BERT based model architecture on C3 challenge. $\lozenge$ is a baseline for bert\_sat, whereas $\blacklozenge$ is a baseline for all other models.}
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Arch}} & \multirow{2}{*}{\textbf{Challenge C3}} & \multicolumn{2}{c|}{CM1} & \multicolumn{2}{c|}{CCHIT} & \multicolumn{2}{c|}{Dronology} & \multicolumn{2}{c|}{PTC} & \multicolumn{2}{c|}{PTC-1} & \multicolumn{2}{c|}{Average Improve} \\ 

\multicolumn{1}{|l|}{} & & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} \\ 

\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering Sat-BERT MSat-BERT}}}
& legacy $\lozenge$ & - & 0.178 & - & 0.010 & - & 0.252 & - & 0.246 & - & 0.177 & - & - \\ 

 & bert\_sat $\blacklozenge$& 0.377 & 0.222 & 0.355 & 0.129 & 0.443 & 0.405 & 0.436 & 0.465 & 0.491 & 0.551 & - & 306.84\% \\ 

 & bert\_mul & 0.369 & 0.249 & 0.352 & 0.098 & 0.431 & 0.437 & 0.420 & 0.442 & 0.431 & 0.469 & -4.33\% & -4.69\% \\ 

 & scibert\_sat & 0.398 & 0.268 & 0.366 & 0.136 & 0.452 & 0.503 & 0.446 & 0.478 & 0.466 & 0.556 & \textbf{1.56\%} & \textbf{10.76\%} \\ 

 & scibert\_mul & 0.370 & 0.273 & 0.346 & 0.130 & 0.432 & 0.516 & 0.423 & 0.450 & 0.440 & 0.510 & -4.04\% & 8.06\% \\ 

 & sebert\_sat & 0.379 & 0.217 & 0.294 & 0.087 & 0.471 & 0.460 & 0.414 & 0.457 & 0.425 & 0.499 & -5.81\% & -6.47\% \\ 

 & sebert\_mul & 0.387 & 0.257 & 0.321 & 0.091 & 0.421 & 0.464 & 0.398 & 0.423 & 0.404 & 0.466 & -7.65\% & -4.68\% \\ 
\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering DSat-BERT DMSat-BERT}}}
& bert\_sat & 0.375 & 0.213 & 0.358 & 0.101 & 0.448 & 0.397 & 0.426 & 0.459 & 0.438 & 0.495 & -2.37\% & -7.84\% \\ 

 & bert\_mul & 0.366 & 0.257 & 0.351 & 0.114 & 0.436 & 0.434 & 0.413 & 0.436 & 0.438 & 0.506 & -4.34\% & -0.66\% \\ 

 & scibert\_sat & 0.395 & 0.237 & 0.361 & 0.176 & 0.474 & 0.502 & 0.424 & 0.466 & 0.444 & 0.512 & \textbf{0.26\%} & \textbf{12.01\%} \\ 

 & scibert\_mul & 0.370 & 0.251 & 0.347 & 0.108 & 0.422 & 0.475 & 0.416 & 0.432 & 0.440 & 0.490 & -4.78\% & -0.76\% \\ 

 & sebert\_sat & 0.383 & 0.238 & 0.324 & 0.102 & 0.457 & 0.439 & 0.382 & 0.418 & 0.386 & 0.449 & -7.58\% & -6.79\% \\ 

 & sebert\_mul & 0.382 & 0.259 & 0.322 & 0.067 & 0.440 & 0.440 & 0.383 & 0.402 & 0.399 & 0.457 & -7.92\% & -10.66\% \\
\hline
\end{tabular}
\end{table*}


% \begin{table*}[t!]
% \centering
% \caption{Performance of various language models leveraging single BERT based model architecture on C3 challenge.}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|} 
% \hline
% \multirow{2}{*}{\textbf{Challenge C3}} & \multicolumn{2}{c|}{CM1} & \multicolumn{2}{c|}{CCHIT} & \multicolumn{2}{c|}{Dronology} & \multicolumn{2}{c|}{PTC} & \multicolumn{2}{c|}{PTC-1} & \multicolumn{2}{c|}{Average Improve} \\ 

%  & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} \\ 
% \hline
% legacy $\lozenge$ & - & 0.178 & - & 0.010 & - & 0.252 & - & 0.246 & - & 0.177 & - & - \\ 

% bert\_sat $\blacklozenge$ & 0.377 & 0.222 & 0.355 & 0.129 & 0.443 & 0.405 & 0.436 & 0.465 & 0.491 & 0.551 & - & 397.65\% \\ 

% bert\_mul & 0.369 & 0.249 & 0.352 & 0.098 & 0.431 & 0.437 & 0.420 & 0.442 & 0.431 & 0.469 & -1.28\% & -2.99\% \\ 

% scibert\_sat & 0.398 & 0.268 & 0.366 & 0.136 & 0.452 & 0.503 & 0.446 & 0.478 & 0.466 & 0.556 & \textbf{3.16\%} & \textbf{11.35\% }\\ 

% scibert\_mul & 0.370 & 0.273 & 0.346 & 0.130 & 0.432 & 0.516 & 0.423 & 0.450 & 0.440 & 0.510 & -1.70\% & 10.92\% \\ 

% sebert\_sat & 0.379 & 0.217 & 0.294 & 0.087 & 0.471 & 0.460 & 0.414 & 0.457 & 0.425 & 0.499 & -4.86\% & -10.06\% \\ 

% sebert\_mul & 0.387 & 0.257 & 0.321 & 0.091 & 0.421 & 0.464 & 0.398 & 0.423 & 0.404 & 0.466 & -2.85\% & -2.87\% \\
% \hline
% \end{tabular}

% \end{table*}

==> tables/ChallengeC1.tex <==
\begin{table*}[t!]
\addtolength{\tabcolsep}{-2.4pt}
\centering
\caption{Performance of BERT-based models leveraging the proposed architectures on C1 challenge --report other results \ap{I think we can remove the average improvement from this tables, and just report the scores. Same on the following tables as well.}}
% \jch{I think L2=Challenge \#1 now.  See figure \ref{tab:C1}. we don't talk about L1 anymore, just C1, C2, C3. So L2=C1, New challenge = C2, and hybrid = C3} against the two datasets - CM1 and Dronology. In this table, we report the performance gains for bert\_sat* over the Legacy Baseline - showing that the naive BERT model alone can significantly outperform the IR-based approaches. However, for the other variants, we consider bert\_sat* in each of the major approaches as our new baseline and report the average performance gain/loss. \jch{Suggest we use this layout for compactness.  I played around with how best to report legacy results, because this way we duplicate them and have to state that they aren't BERT related.  I think that is OK.  It is a tradeoff against space.}} 
\label{tab:C1}
	\centering
\begin{tabular}{|c|l|cc|cc|cc|cc|cc|cc|cc|cc|} \hline
\multicolumn{2}{|c|}{}& \multicolumn{8}{c|}{Sat-BERT \& MSat-BERT}& \multicolumn{8}{c|}{DSat-BERT \& DMSat-BERT}\\ \cline{3-18}
 \multicolumn{2}{|c|}{{\bf Challenge C1}} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300}& \multicolumn{2}{c|}{500}  & \multicolumn{2}{c|}{Avg Improve.} & \multicolumn{2}{c|}{100}& \multicolumn{2}{c|}{300}& \multicolumn{2}{c|}{500}  & \multicolumn{2}{c|}{Avg Improve.}\\ 
\multicolumn{2}{|c|}{}& \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP}&\multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} \\ 
\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CM1}}}

& legacy $\lozenge$ & 0.115 & 0.199 & 0.058 & 0.167 & 0.046 & 0.166 & \multicolumn{1}{l}{–} & \multicolumn{1}{l|}{–} & 0.115 & 0.199 & 0.058 & 0.167 & 0.046 & 0.166 & \multicolumn{1}{l}{–} & \multicolumn{1}{l|}{–} \\ 

 & bert\_sat $\blacklozenge$ & 0.211 & 0.264 & 0.142 & 0.189 & 0.137 & 0.164 & 143.46\% & 14.69\% & 0.247 & 0.303 & 0.190 & 0.192 & 0.118 & 0.112 & 167.82\% & 11.35\% \\ 
 & bert\_mul & 0.253 & 0.346 & 0.222 & 0.263 & 0.175 & 0.208 & 34.65\% & 32.34\% & 0.263 & 0.339 & 0.221 & 0.261 & 0.178 & 0.205 & 24.79\% & 43.79\% \\ 

 & scibert\_sat & 0.225 & 0.265 & 0.270 & 0.262 & 0.269 & 0.263 & 64.38\% & 33.26\% & 0.286 & 0.328 & 0.223 & 0.243 & 0.237 & 0.267 & 44.91\% & 58.07\% \\ 

 & scibert\_mul & 0.319 & 0.338 & 0.255 & 0.274 & 0.249 & 0.253 & 70.94\% & 42.62\% & 0.297 & 0.377 & 0.254 & 0.295 & 0.246 & 0.251 & 54.36\% & 67.81\% \\ 

 & sebert\_sat & 0.318 & 0.338 & 0.207 & 0.282 & 0.231 & 0.215 & 55.06\% & 36.18\% & 0.280 & 0.369 & 0.250 & 0.245 & 0.190 & 0.185 & 35.35\% & 38.58\% \\ 

 & sebert\_mul & 0.351 & 0.388 & 0.249 & 0.322 & 0.295 & 0.367 & 85.74\% & 80.33\% & 0.376 & 0.397 & 0.257 & 0.286 & 0.235 & 0.256 & 62.39\% & 69.77\% \\ 
\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CCHIT}}}

& legacy $\lozenge$ & 0.064 & 0.016 & 0.025 & 0.008 & 0.019 & 0.007 & \multicolumn{1}{l}{–} & \multicolumn{1}{l|}{–} & 0.064 & 0.016 & 0.025 & 0.008 & 0.019 & 0.007 & \multicolumn{1}{l}{–} & \multicolumn{1}{l|}{–} \\ 

 & bert\_sat $\blacklozenge$ & 0.211 & 0.135 & 0.162 & 0.114 & 0.151 & 0.066 & 492.25\% & 971.65\% & 0.238 & 0.220 & 0.235 & 0.165 & 0.190 & 0.167 & 670.07\% & 1841.94\% \\ 

 & bert\_mul & 0.275 & 0.179 & 0.228 & 0.179 & 0.195 & 0.180 & 33.03\% & 87.01\% & 0.274 & 0.230 & 0.194 & 0.109 & 0.198 & 0.114 & 0.82\% & -20.38\% \\ 

 & scibert\_sat & 0.241 & 0.351 & 0.266 & 0.217 & 0.279 & 0.293 & 54.17\% & 197.31\% & 0.232 & 0.284 & 0.197 & 0.281 & 0.245 & 0.248 & 3.58\% & 49.24\% \\ 

 & scibert\_mul & 0.294 & 0.263 & 0.257 & 0.207 & 0.259 & 0.203 & 56.25\% & 127.57\% & 0.241 & 0.277 & 0.241 & 0.221 & 0.247 & 0.157 & 11.36\% & 18.01\% \\ 

 & sebert\_sat & 0.203 & 0.138 & 0.108 & 0.092 & 0.173 & 0.072 & -7.88\% & -2.87\% & 0.236 & 0.172 & 0.193 & 0.102 & 0.122 & 0.094 & -18.03\% & -34.66\% \\ 

 & sebert\_mul & 0.241 & 0.196 & 0.125 & 0.083 & 0.150 & 0.047 & -3.12\% & -3.93\% & 0.203 & 0.166 & 0.218 & 0.166 & 0.210 & 0.164 & -3.65\% & -8.42\% \\ 

\hline



\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering Dronology}}}
& legacy $\lozenge$ & 0.114 & 0.293 & 0.042 & 0.234 & 0.028 & 0.233 & \multicolumn{1}{l}{–} & \multicolumn{1}{l|}{–} & 0.114 & 0.293 & 0.042 & 0.234 & 0.028 & 0.233 & \multicolumn{1}{l}{–} & \multicolumn{1}{l|}{–} \\ 

 & bert\_sat $\blacklozenge$ & 0.538 & 0.678 & 0.374 & 0.488 & 0.358 & 0.439 & 784.59\% & 109.68\% & 0.550 & 0.710 & 0.405 & 0.562 & 0.394 & 0.490 & 855.71\% & 131.16\% \\ 

 & bert\_mul & 0.469 & 0.664 & 0.462 & 0.576 & 0.395 & 0.457 & 6.98\% & 6.66\% & 0.563 & 0.705 & 0.383 & 0.463 & 0.403 & 0.482 & -0.29\% & -6.66\% \\ 

 & scibert\_sat & 0.534 & 0.687 & 0.435 & 0.561 & 0.450 & 0.589 & 13.78\% & 16.79\% & 0.510 & 0.630 & 0.471 & 0.561 & 0.339 & 0.399 & -1.67\% & -10.00\% \\ 

 & scibert\_mul & 0.531 & 0.731 & 0.492 & 0.636 & 0.411 & 0.542 & 15.04\% & 20.53\% & 0.553 & 0.724 & 0.491 & 0.600 & 0.434 & 0.488 & 10.73\% & 2.84\% \\ 

 & sebert\_sat & 0.633 & 0.792 & 0.498 & 0.604 & 0.491 & 0.619 & 29.39\% & 27.19\% & 0.532 & 0.649 & 0.491 & 0.591 & 0.506 & 0.548 & 15.54\% & 2.77\% \\ 

 & sebert\_mul & 0.603 & 0.798 & 0.499 & 0.508 & 0.458 & 0.573 & 24.53\% & 17.45\% & 0.597 & 0.653 & 0.527 & 0.615 & 0.504 & 0.552 & 22.25\% & 4.67\% \\ 
\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering PTC}}}

& legacy $\lozenge$ & 0.158 & 0.310 & 0.069 & 0.214 & 0.047 & 0.210 & \multicolumn{1}{l}{–} & \multicolumn{1}{l|}{–} & 0.158 & 0.310 & 0.069 & 0.214 & 0.047 & 0.210 & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ 

 & bert\_sat $\blacklozenge$ & 0.549 & 0.607 & 0.465 & 0.525 & 0.404 & 0.468 & 527.13\% & 121.42\% & 0.514 & 0.635 & 0.381 & 0.497 & 0.403 & 0.470 & 478.32\% & 120.31\% \\ 
 & bert\_mul & 0.539 & 0.637 & 0.463 & 0.555 & 0.384 & 0.480 & -2.45\% & 4.39\% & 0.570 & 0.638 & 0.434 & 0.508 & 0.399 & 0.508 & 7.92\% & 3.59\% \\ 

 & scibert\_sat & 0.594 & 0.668 & 0.496 & 0.569 & 0.438 & 0.537 & 7.74\% & 10.98\% & 0.589 & 0.648 & 0.435 & 0.521 & 0.438 & 0.486 & 12.48\% & 3.46\% \\ 

 & scibert\_mul & 0.585 & 0.663 & 0.462 & 0.534 & 0.449 & 0.521 & 5.68\% & 7.35\% & 0.585 & 0.661 & 0.450 & 0.540 & 0.438 & 0.511 & 13.53\% & 7.20\% \\ 

 & sebert\_sat & 0.588 & 0.693 & 0.426 & 0.519 & 0.354 & 0.467 & -4.54\% & 4.28\% & 0.501 & 0.618 & 0.330 & 0.449 & 0.368 & 0.512 & -8.19\% & -1.14\% \\ 

 & sebert\_mul & 0.577 & 0.639 & 0.451 & 0.546 & 0.383 & 0.480 & -1.05\% & 3.92\% & 0.500 & 0.604 & 0.394 & 0.532 & 0.368 & 0.402 & -2.73\% & -4.14\% \\ 


\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering PTC-1}}}
& legacy $\lozenge$ & 0.164 & 0.254 & 0.107 & 0.205 & 0.097 & 0.205 & \multicolumn{1}{l}{–} & \multicolumn{1}{l|}{–} & 0.164 & 0.254 & 0.107 & 0.205 & 0.097 & 0.205 & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ 

 & bert\_sat $\blacklozenge$ & 0.519 & 0.632 & 0.485 & 0.550 & 0.448 & 0.556 & 309.43\% & 162.67\% & 0.488 & 0.613 & 0.453 & 0.553 & 0.428 & 0.544 & 286.42\% & 158.72\% \\ 
 
 & bert\_mul & 0.533 & 0.619 & 0.479 & 0.544 & 0.469 & 0.528 & 1.98\% & -2.74\% & 0.553 & 0.627 & 0.429 & 0.558 & 0.444 & 0.503 & 3.92\% & -1.46\% \\ 

 & scibert\_sat & 0.564 & 0.640 & 0.497 & 0.571 & 0.510 & 0.584 & 8.34\% & 3.42\% & 0.554 & 0.639 & 0.484 & 0.560 & 0.493 & 0.557 & 11.41\% & 2.61\% \\ 

 & scibert\_mul & 0.556 & 0.616 & 0.424 & 0.498 & 0.463 & 0.511 & -0.73\% & -6.63\% & 0.578 & 0.647 & 0.488 & 0.573 & 0.462 & 0.513 & 10.46\% & 1.02\% \\ 

 & sebert\_sat & 0.459 & 0.551 & 0.392 & 0.482 & 0.406 & 0.484 & -13.36\% & -12.71\% & 0.441 & 0.512 & 0.295 & 0.378 & 0.371 & 0.465 & -17.98\% & -20.20\% \\ 

 & sebert\_mul & 0.486 & 0.558 & 0.395 & 0.462 & 0.325 & 0.387 & -17.47\% & -19.37\% & 0.464 & 0.548 & 0.346 & 0.388 & 0.381 & 0.422 & -17.58\% & -26.28\% \\
\hline


\end{tabular}

$\blacklozenge$ = Baseline for the BERT-based models, Variants of single task variants are suffixed as \_sat, whereas the multitask variants are suffixed as \_mul.\\
$\lozenge$=Legacy results using VSM without use of BERT models.
\end{table*}


% \usepackage{colortbl}







==> tables/ChallengeC2.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table*}[t!]
\centering
\caption{Performance of BERT-based models (Sat-BERT \& MSat-BERT) leveraging the proposed architectures on C2 challenge} 
\scalebox{0.9}{
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
 \multicolumn{2}{|c|}{{\bf Challenge C2}} &\multicolumn{2}{c|}{2} & \multicolumn{2}{c|}{3} & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{5} & \multicolumn{2}{c|}{6} & \multicolumn{2}{c|}{7} & \multicolumn{2}{c|}{9} & \multicolumn{2}{c|}{\bf Avg Improve.} \\

\multicolumn{2}{|c|}{}& \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP \\ 

\hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CM-1}}} & bert\_sat & 0.955 & 0.867 & 0.910 & 0.803 & 0.774 & 0.563 & 0.859 & 0.815 & 0.652 & 0.394 & - & - & - & - & 144.33\% & 532.20\% \\ 
 & bert\_mul & 0.868 & 0.656 & 0.971 & 0.933 & 0.908 & 0.813 & 0.909 & 0.767 & 0.669 & 0.487 & - & - & - & - & 4.67\% & 10.79\% \\ 

 & scibert\_sat & 0.943 & 0.867 & 0.933 & 0.867 & 0.983 & 0.950 & 0.943 & 0.867 & 0.720 & 0.515 & - & - & - & - & 9.67\% & 22.78\% \\ 

 & scibert\_mul & 0.959 & 0.889 & 0.963 & 0.925 & 0.943 & 0.867 & 0.967 & 0.900 & 0.943 & 0.867 & - & - & - & - & 17.00\% & 40.47\% \\ 

 & sebert\_sat & 0.932 & 0.833 & 0.971 & 0.933 & 0.963 & 0.925 & 1.000 & 1.000 & 0.834 & 0.695 & - & - & - & - & 14.58\% & 35.21\% \\ 

 & sebert\_mul & 0.882 & 0.711 & 0.946 & 0.914 & 0.929 & 0.864 & 0.909 & 0.767 & 0.699 & 0.472 & - & - & - & - & 5.85\% & 12.67\% \\ 
\hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CCHIT}}}
 & bert\_sat & 0.876 & 0.667 & 1.000 & 1.000 & 0.779 & 0.557 & 0.834 & 0.695 & 0.619 & 0.512 & 0.783 & 0.658 & 0.878 & 0.740 & 1058.85\% & 4381.79\% \\ 

 & bert\_mul & 0.852 & 0.633 & 0.783 & 0.579 & 0.714 & 0.630 & 1.000 & 1.000 & 0.615 & 0.511 & 0.368 & 0.243 & 0.738 & 0.553 & -11.79\% & -11.25\% \\ 

 & scibert\_sat & 0.938 & 0.833 & 0.933 & 0.800 & 0.900 & 0.833 & 0.967 & 0.900 & 0.871 & 0.820 & 0.805 & 0.620 & 0.871 & 0.820 & 10.65\% & 21.34\% \\ 

 & scibert\_mul & 0.938 & 0.833 & 0.967 & 0.900 & 1.000 & 1.000 & 0.943 & 0.867 & 1.000 & 1.000 & 0.753 & 0.650 & 0.762 & 0.580 & 12.80\% & 27.40\% \\ 

 & sebert\_sat & 0.886 & 0.733 & 0.911 & 0.840 & 0.814 & 0.687 & 1.000 & 1.000 & 0.786 & 0.704 & 0.589 & 0.455 & 0.598 & 0.462 & -1.87\% & 4.33\% \\ 

 & sebert\_mul & 0.893 & 0.750 & 0.847 & 0.675 & 0.816 & 0.767 & 1.000 & 1.000 & 1.000 & 1.000 & 0.757 & 0.604 & 0.693 & 0.571 & 6.90\% & 17.98\% \\ 
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering Dronology}}}
& bert\_sat & 0.983 & 0.950 & 0.967 & 0.900 & 0.967 & 0.900 & 1.000 & 1.000 & - & - & - & - & 0.254 & 0.076 & 635.72\% & 1454.70\% \\ 

 & bert\_mul & 0.971 & 0.933 & 0.900 & 0.833 & 1.000 & 1.000 & 0.911 & 0.840 & - & - & - & - & 0.176 & 0.074 & -8.85\% & -3.50\% \\ 

 & scibert\_sat & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 0.900 & 0.700 & - & - & - & - & 0.753 & 0.577 & 38.90\% & 130.73\% \\ 

 & scibert\_mul & 0.971 & 0.933 & 1.000 & 1.000 & 0.911 & 0.840 & 0.750 & 0.565 & - & - & - & - & 0.526 & 0.443 & 15.63\% & 87.90\% \\ 

 & sebert\_sat & 1.000 & 1.000 & 1.000 & 1.000 & 0.817 & 0.625 & 0.769 & 0.572 & - & - & - & - & 0.624 & 0.605 & 22.34\% & 127.13\% \\ 

 & sebert\_mul & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 0.800 & 0.667 & - & - & - & - & 0.296 & 0.134 & 1.02\% & 13.86\% \\ 
\hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering PTC}}}
& bert\_sat & 0.990 & 0.971 & 0.917 & 0.808 & 0.858 & 0.650 & 0.502 & 0.189 & 0.560 & 0.333 & - & - & - & - & 89.93\% & 281.07\% \\ 

 & bert\_mul & 0.981 & 0.943 & 0.983 & 0.950 & 0.850 & 0.700 & 0.637 & 0.470 & 0.817 & 0.713 & - & - & - & - & 15.60\% & 57.02\% \\ 

 & scibert\_sat & 1.000 & 1.000 & 1.000 & 1.000 & 0.892 & 0.750 & 0.684 & 0.395 & 0.584 & 0.450 & - & - & - & - & 10.87\% & 37.29\% \\ 

 & scibert\_mul & 0.990 & 0.971 & 0.983 & 0.950 & 0.967 & 0.900 & 0.698 & 0.429 & 0.727 & 0.635 & - & - & - & - & 17.73\% & 54.72\% \\ 

 & sebert\_sat & 1.000 & 1.000 & 0.967 & 0.900 & 0.933 & 0.800 & 0.925 & 0.850 & 0.555 & 0.359 & - & - & - & - & 19.71\% & 78.92\% \\ 

 & sebert\_mul & 0.987 & 0.967 & 0.938 & 0.833 & 0.858 & 0.650 & 0.734 & 0.520 & 0.657 & 0.410 & - & - & - & - & 13.07\% & 40.14\% \\ 
\hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering PTC-1}}} 
& bert\_sat & 1.000 & 1.000 & 0.819 & 0.533 & 0.721 & 0.545 & - & - & - & - & - & - & - & - & 21.08\% & 79.65\% \\ 

 & bert\_mul & 1.000 & 1.000 & 0.958 & 0.875 & 0.906 & 0.813 & - & - & - & - & - & - & - & - & 14.22\% & 37.72\% \\ 

 & scibert\_sat & 1.000 & 1.000 & 0.967 & 0.900 & 0.733 & 0.552 & - & - & - & - & - & - & - & - & 6.56\% & 23.32\% \\ 

 & scibert\_mul & 1.000 & 1.000 & 0.852 & 0.633 & 0.809 & 0.600 & - & - & - & - & - & - & - & - & 5.43\% & 9.61\% \\ 

 & sebert\_sat & 1.000 & 1.000 & 0.933 & 0.800 & 0.720 & 0.515 & - & - & - & - & - & - & - & - & 4.57\% & 14.83\% \\ 

 & sebert\_mul & 1.000 & 1.000 & 0.909 & 0.767 & 0.670 & 0.385 & - & - & - & - & - & - & - & - & 1.31\% & 4.81\% \\
\hline
\end{tabular}}
\end{table*}

==> tables/ChallengeC2Dual.tex <==

\begin{table*}[t!]
\centering
\caption{Performance of BERT-based models (DSat-BERT \& DMSat-BERT) leveraging the proposed architectures on C2 challenge} 
\scalebox{0.9}{
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
 \multicolumn{2}{|c|}{{\bf Challenge C2}} &\multicolumn{2}{c|}{2} & \multicolumn{2}{c|}{3} & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{5} & \multicolumn{2}{c|}{6} & \multicolumn{2}{c|}{7} & \multicolumn{2}{c|}{9} & \multicolumn{2}{c|}{\bf Avg Improve.} \\

\multicolumn{2}{|c|}{}& \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP & \multicolumn{1}{c}{F2} & MAP \\ 

\hline
%CM1
% \multirow{30}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CM-1}}}&
\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CM-1}}} & bert\_sat    & 0.936 & 0.822 & 0.913 & 0.842 & 0.759 & 0.593 & 0.909 & 0.767 & 0.487 & 0.303 & -     & -     & -     & -     & 123.67\%  & 468.87\%   \\ 

&bert\_mul    & 0.933 & 0.800 & 0.929 & 0.825 & 0.912 & 0.814 & 0.741 & 0.554 & 0.617 & 0.466 & -     & -     & -     & -     & 5.98\%    & 11.68\%    \\ 

&scibert\_sat & 0.978 & 0.933 & 0.946 & 0.914 & 0.938 & 0.833 & 0.900 & 0.833 & 0.657 & 0.482 & -     & -     & -     & -     & 13.12\%   & 26.01\%    \\ 

&scibert\_mul & 0.978 & 0.933 & 0.927 & 0.853 & 0.904 & 0.838 & 0.786 & 0.589 & 0.610 & 0.372 & -     & -     & -     & -     & 7.41\%    & 11.11\%    \\ 

&sebert\_sat  & 0.948 & 0.856 & 0.963 & 0.925 & 0.938 & 0.833 & 0.886 & 0.733 & 0.637 & 0.429 & -     & -     & -     & -     & 11.71\%   & 18.32\%    \\ 

&sebert\_mul  & 0.951 & 0.878 & 0.971 & 0.933 & 0.917 & 0.808 & 0.833 & 0.633 & 0.420 & 0.273 & -     & -     & -     & -     & 1.35\%    & 5.28\%     \\ 
\hline

%CCHIT
\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CCHIT}}}
&bert\_sat    & 0.967 & 0.900 & 0.850 & 0.700 & 0.933 & 0.800 & 0.925 & 0.850 & 0.753 & 0.489 & 0.967 & 0.900 & 0.828 & 0.600 & 1053.12\% & 3826.31\%  \\ 

&bert\_mul    & 0.967 & 0.900 & 0.967 & 0.900 & 1.000 & 1.000 & 0.821 & 0.607 & 0.684 & 0.621 & 0.445 & 0.318 & 0.502 & 0.296 & -13.28\%  & -9.08\%    \\ 

&scibert\_sat & 0.950 & 0.850 & 0.819 & 0.533 & 1.000 & 1.000 & 1.000 & 1.000 & 0.871 & 0.820 & 0.698 & 0.538 & 0.537 & 0.304 & -5.35\%   & -1.23\%    \\ 

&scibert\_mul & 0.983 & 0.950 & 0.967 & 0.900 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 0.733 & 0.636 & 0.909 & 0.767 & 7.02\%    & 25.69\%    \\ 

&sebert\_sat  & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 0.640 & 0.491 & 0.640 & 0.390 & 1.80\%    & 17.25\%    \\ 

&sebert\_mul  & 0.983 & 0.950 & 1.000 & 1.000 & 0.909 & 0.767 & 0.836 & 0.808 & 1.000 & 1.000 & 0.810 & 0.802 & 0.584 & 0.450 & -0.82\%   & 15.43\%    \\ 
\hline

%DRONOLOGY
\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering Dronology}}}
&bert\_sat    & 0.983 & 0.950 & 0.967 & 0.900 & 0.858 & 0.650 & 0.737 & 0.561 & -     & -     & -     & -     & 0.131 & 0.033 & 354.73\%  & 771.26\%   \\ 

&bert\_mul    & 1.000 & 1.000 & 0.943 & 0.867 & 0.843 & 0.567 & 0.758 & 0.568 & -     & -     & -     & -     & 0.107 & 0.025 & -3.64\%   & -6.82\%    \\ 

&scibert\_sat & 0.967 & 0.900 & 0.967 & 0.900 & 0.789 & 0.580 & 0.810 & 0.622 & -     & -     & -     & -     & 0.458 & 0.413 & 49.90\%   & 226.82\%   \\ 

&scibert\_mul & 1.000 & 1.000 & 1.000 & 1.000 & 0.878 & 0.740 & 0.821 & 0.607 & -     & -     & -     & -     & 0.541 & 0.440 & 66.38\%   & 252.18\%   \\ 

&sebert\_sat  & 1.000 & 1.000 & 0.800 & 0.595 & 0.854 & 0.707 & 0.809 & 0.600 & -     & -     & -     & -     & 0.484 & 0.421 & 52.63\%   & 230.12\%   \\ 

&sebert\_mul  & 1.000 & 1.000 & 1.000 & 1.000 & 0.876 & 0.667 & 0.804 & 0.709 & -     & -     & -     & -     & 0.339 & 0.246 & 35.07\%   & 136.78\%   \\ 
\hline

%PTC

\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering PTC}}}
&bert\_sat    & 0.958 & 0.881 & 0.818 & 0.567 & 0.854 & 0.707 & 0.321 & 0.091 & 0.174 & 0.041 & -     & -     & -     & -     & 24.49\%   & 82.20\%    \\ 

&bert\_mul    & 0.976 & 0.929 & 0.877 & 0.703 & 0.925 & 0.850 & 0.446 & 0.147 & 0.406 & 0.253 & -     & -     & -     & -     & 37.87\%   & 125.62\%   \\ 

&scibert\_sat & 0.986 & 0.957 & 0.875 & 0.700 & 0.824 & 0.629 & 0.506 & 0.299 & 0.679 & 0.619 & -     & -     & -     & -     & 70.66\%   & 331.60\%   \\ 

&scibert\_mul & 0.971 & 0.914 & 0.893 & 0.717 & 0.925 & 0.850 & 0.356 & 0.102 & 0.613 & 0.393 & -     & -     & -     & -     & 56.33\%   & 184.04\%   \\ 

&sebert\_sat  & 0.995 & 0.986 & 0.884 & 0.708 & 0.876 & 0.667 & 0.439 & 0.176 & 0.343 & 0.143 & -     & -     & -     & -     & 29.58\%   & 74.98\%    \\ 

&sebert\_mul  & 0.995 & 0.986 & 0.950 & 0.850 & 0.819 & 0.533 & 0.503 & 0.195 & 0.319 & 0.113 & -     & -     & -     & -     & 31.11\%   & 65.64\%    \\ 
\hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering PTC-1}}} 
&bert\_sat    & 0.994 & 0.983 & 0.900 & 0.700 & 0.802 & 0.672 & -     & -     & -     & -     & -     & -     & -     & -     & 29.58\%   & 113.31\%   \\ 

&bert\_mul    & 0.994 & 0.983 & 0.967 & 0.900 & 0.817 & 0.600 & -     & -     & -     & -     & -     & -     & -     & -     & 3.08\%    & 5.94\%     \\ 

& scibert\_sat & 1.000 & 1.000 & 0.933 & 0.800 & 0.909 & 0.767 & -     & -     & -     & -     & -     & -     & -     & -     & 5.89\%    & 10.01\%    \\ 

& scibert\_mul & 1.000 & 1.000 & 0.943 & 0.867 & 0.925 & 0.850 & -     & -     & -     & -     & -     & -     & -     & -     & 6.89\%    & 17.32\%    \\ 

&sebert\_sat  & 0.994 & 0.983 & 1.000 & 1.000 & 0.909 & 0.767 & -     & -     & -     & -     & -     & -     & -     & -     & 8.18\%    & 18.97\%    \\ 

&sebert\_mul  & 0.994 & 0.983 & 1.000 & 1.000 & 0.826 & 0.692 & -     & -     & -     & -     & -     & -     & -     & -     & 4.72\%    & 15.25\%    \\
\hline
\end{tabular}}
\end{table*}



==> tables/ChallengeC3.tex <==


\begin{table*}[t!]
\addtolength{\tabcolsep}{-2.7pt}
\centering
\caption{Performance of BERT-based models leveraging the proposed architectures on C3 challenge} 
\label{tab:C3}
	\centering
% \addtolength{\tabcolsep}{-1pt}
\begin{tabular}{|c|l|cc|cc|cc|cc|cc|cc|cc|cc|} \hline
\multicolumn{2}{|c|}{}& \multicolumn{8}{c|}{Sat-BERT \& MSat-BERT}& \multicolumn{8}{c|}{DSat-BERT \& DMSat-BERT}\\ \cline{3-18}
 \multicolumn{2}{|c|}{{\bf Challenge C3}} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{300}& \multicolumn{2}{c|}{500}  & \multicolumn{2}{c|}{Avg Improve.} & \multicolumn{2}{c|}{100}& \multicolumn{2}{c|}{300}& \multicolumn{2}{c|}{500}  & \multicolumn{2}{c|}{Avg Improve.}\\ 
\multicolumn{2}{|c|}{}& \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{MAP}&\multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{MAP} \\ 


\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CM-1}}} 

&legacy $\lozenge$  & -     & 0.200 & -     & 0.167 & -     & 0.166 & -       & -       & -     & 0.200 & -     & 0.167 & -     & 0.166 & -       & \multicolumn{1}{l|}{-}  \\ 

& bert\_sat $\blacklozenge$ & 0.380 & 0.334 & 0.368 & 0.167 & 0.382 & 0.164 & -       & 21.78\% & 0.377 & 0.295 & 0.367 & 0.193 & 0.380 & 0.152 & -       & 17.93\%                 \\ 

& bert\_mul   & 0.402 & 0.310 & 0.346 & 0.243 & 0.358 & 0.193 & -2.16\% & 18.62\% & 0.399 & 0.367 & 0.355 & 0.187 & 0.345 & 0.217 & -2.21\% & 21.49\%                 \\ 

& scibert\_sat & 0.424 & 0.365 & 0.380 & 0.200 & 0.390 & 0.238 & 5.64\%  & 24.71\% & 0.395 & 0.286 & 0.405 & 0.237 & 0.386 & 0.187 & 5.57\%  & 14.23\%                 \\ 

& scibert\_mul & 0.397 & 0.313 & 0.356 & 0.293 & 0.357 & 0.212 & -1.78\% & 32.68\% & 0.403 & 0.289 & 0.355 & 0.257 & 0.352 & 0.208 & -1.25\% & 22.72\%                 \\ 

& sebert\_sat & 0.369 & 0.253 & 0.380 & 0.181 & 0.387 & 0.218 & 0.56\%  & 5.64\%  & 0.367 & 0.310 & 0.394 & 0.223 & 0.388 & 0.180 & 2.27\%  & 13.02\%                 \\ 

& sebert\_mul & 0.412 & 0.333 & 0.380 & 0.238 & 0.370 & 0.201 & 2.85\%  & 21.58\% & 0.400 & 0.356 & 0.375 & 0.224 & 0.371 & 0.196 & 1.97\%  & 21.82\%                 \\

\hline

%%%% CCHIT
\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering CCHIT}}} 

& legacy $\lozenge$ & - & 0.016 & - & 0.008 & - & 0.007 & - & - & - & 0.016 & - & 0.008 & - & 0.007 & - & \multicolumn{1}{l|}{-} \\ 

 & bert\_sat $\blacklozenge$ & 0.354 & 0.199 & 0.362 & 0.099 & 0.350 & 0.089 & - & 1150.71\% & 0.337 & 0.143 & 0.368 & 0.085 & 0.367 & 0.074 & - & 905.14\% \\ 

 & bert\_mul & 0.337 & 0.103 & 0.379 & 0.113 & 0.341 & 0.078 & -0.85\% & -15.19\% & 0.365 & 0.164 & 0.332 & 0.057 & 0.356 & 0.119 & -1.60\% & 14.40\% \\ 

 & scibert\_sat & 0.362 & 0.206 & 0.393 & 0.151 & 0.345 & 0.050 & 3.11\% & 4.26\% & 0.352 & 0.287 & 0.360 & 0.097 & 0.372 & 0.143 & 1.10\% & 69.34\% \\ 

 & scibert\_mul & 0.330 & 0.128 & 0.371 & 0.145 & 0.338 & 0.116 & -2.56\% & 13.78\% & 0.342 & 0.125 & 0.342 & 0.133 & 0.358 & 0.066 & -2.86\% & 11.04\% \\ 

 & sebert\_sat & 0.230 & 0.145 & 0.318 & 0.090 & 0.334 & 0.026 & -17.22\% & -35.90\% & 0.310 & 0.141 & 0.334 & 0.097 & 0.327 & 0.068 & -9.39\% & 1.40\% \\ 

 & sebert\_mul & 0.282 & 0.125 & 0.352 & 0.114 & 0.327 & 0.033 & -9.80\% & -28.02\% & 0.270 & 0.094 & 0.326 & 0.053 & 0.371 & 0.054 & -10.14\% & -32.76\% \\ 
\hline

%%%% Dronology


\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering Dronology}}} 

& legacy $\lozenge$ & - & 0.270 & - & 0.254 & - & 0.233 & - & - & - & 0.270 & - & 0.254 & - & 0.233 & - & \multicolumn{1}{l|}{-} \\ 

& bert\_sat $\blacklozengelozenge$ & 0.466 & 0.508 & 0.431 & 0.366 & 0.432 & 0.341 & - & 59.61\% & 0.483 & 0.511 & 0.440 & 0.338 & 0.420 & 0.343 & - & 56.68\% \\\ 

&bert\_mul                             & 0.468 & 0.501 & 0.405 & 0.408 & 0.420 & 0.403 & -2.79\% & 9.43\%  & 0.489 & 0.518 & 0.407 & 0.411 & 0.413 & 0.372 & -2.64\% & 10.47\% \\  

&scibert\_sat                          & 0.450 & 0.523 & 0.442 & 0.486 & 0.463 & 0.500 & 2.10\%  & 27.46\% & 0.482 & 0.542 & 0.477 & 0.470 & 0.463 & 0.495 & 6.15\%  & 29.81\%  \\ 

&scibert\_mul                          & 0.487 & 0.606 & 0.388 & 0.488 & 0.422 & 0.454 & -2.60\% & 28.59\% & 0.429 & 0.565 & 0.440 & 0.456 & 0.397 & 0.403 & -5.55\% & 20.99\% \\ 

&sebert\_sat                           & 0.470 & 0.569 & 0.477 & 0.408 & 0.466 & 0.402 & 6.47\%  & 13.79\% & 0.474 & 0.505 & 0.462 & 0.394 & 0.434 & 0.417 & 2.16\%  & 12.32\%  \\ 

&sebert\_mul                           & 0.439 & 0.550 & 0.396 & 0.420 & 0.429 & 0.421 & -4.87\% & 15.49\% & 0.477 & 0.522 & 0.439 & 0.367 & 0.403 & 0.430 & -1.84\% & 12.03\%  \\   



% %%%% WorldVista/CCHITT
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering WorldVista}}} &legacy$\lozenge$ &&&&&&&&&&&&&&&&\\
% &bert\_sat $\blacklozenge$  &&&&&&&&&&&&&&&&\\ 

% &bert\_mul   &&&&&&&&&&&&&&&&\\

% &scibert\_sat   &&&&&&&&&&&&&&&&\\

% &scibert\_mul    &&&&&&&&&&&&&&&&\\

%  &sebert\_sat   &&&&&&&&&&&&&&&&\\

% & sebert\_mul   &&&&&&&&&&&&&&&&\\
% \cline{1-18}


%---------------------------------------------------------------------%
%---------------------------------------------------------------------%
%---------------------------------------------------------------------%



% \usepackage{multirow}
% \usepackage{colortbl}


% \usepackage{multirow}
% \usepackage{colortbl}


\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.8cm}{\centering PTC}}} 

& legacy $\lozenge$ & - & 0.314 & - & 0.215 & - & 0.210 & - & - & - & 0.314 & - & 0.215 & - & 0.210 & - & \multicolumn{1}{l|}{-} \\ 

 & bert\_sat $\blacklozenge$ & 0.475 & 0.562 & 0.419 & 0.411 & 0.414 & 0.422 & - & \multicolumn{1}{l|}{90.30\%} & 0.477 & 0.570 & 0.419 & 0.403 & 0.384 & 0.403 & - & 86.91\% \\ 

 & bert\_mul & 0.475 & 0.574 & 0.402 & 0.392 & 0.382 & 0.359 & -3.91\% & \multicolumn{1}{l|}{-5.75\%} & 0.465 & 0.548 & 0.396 & 0.393 & 0.378 & 0.369 & -3.17\% & -4.96\% \\ 

 & scibert\_sat & 0.482 & 0.541 & 0.446 & 0.459 & 0.410 & 0.433 & 2.29\% & \multicolumn{1}{l|}{3.54\%} & 0.459 & 0.568 & 0.413 & 0.418 & 0.401 & 0.411 & -0.19\% & 1.81\% \\ 

 & scibert\_mul & 0.470 & 0.568 & 0.408 & 0.406 & 0.390 & 0.375 & -3.15\% & \multicolumn{1}{l|}{-3.70\%} & 0.460 & 0.543 & 0.388 & 0.371 & 0.400 & 0.382 & -2.24\% & -5.97\% \\ 

 & sebert\_sat & 0.448 & 0.564 & 0.421 & 0.402 & 0.373 & 0.404 & -5.07\% & \multicolumn{1}{l|}{-2.00\%} & 0.395 & 0.493 & 0.375 & 0.377 & 0.377 & 0.384 & -9.82\% & -8.18\% \\ 

 & sebert\_mul & 0.441 & 0.505 & 0.384 & 0.426 & 0.371 & 0.338 & -8.68\% & \multicolumn{1}{l|}{-8.74\%} & 0.403 & 0.487 & 0.373 & 0.367 & 0.372 & 0.352 & -9.84\% & -12.06\% \\ 
\hline



\multicolumn{1}{|c|}{\multirow{7}{*}{PTC-1}} 

& legacy $\lozenge$ & - & 0.205 & - & 0.162 & - & 0.162 & - & \multicolumn{1}{l|}{} & - & 0.205 & - & 0.162 & - & 0.162 & - & \multicolumn{1}{l|}{-} \\ 

& bert\_sat $\blacklozenge$ & 0.492 & 0.588 & 0.492 & 0.548 & 0.491 & 0.517 & - & \multicolumn{1}{l|}{214.39\%} & 0.473 & 0.554 & 0.419 & 0.469 & 0.422 & 0.461 & - & 181.08\% \\ 

& bert\_mul & 0.470 & 0.541 & 0.421 & 0.461 & 0.403 & 0.406 & -12.27\% & \multicolumn{1}{l|}{-15.12\%} & 0.462 & 0.566 & 0.431 & 0.469 & 0.419 & 0.482 & 0.01\% & 2.26\% \\ 

& scibert\_sat & 0.480 & 0.616 & 0.460 & 0.527 & 0.457 & 0.526 & -5.23\% & \multicolumn{1}{l|}{0.82\%} & 0.485 & 0.568 & 0.417 & 0.499 & 0.429 & 0.469 & 1.30\% & 3.53\% \\ 

& scibert\_mul & 0.466 & 0.575 & 0.417 & 0.488 & 0.437 & 0.466 & -10.44\% & \multicolumn{1}{l|}{-7.69\%} & 0.470 & 0.578 & 0.429 & 0.476 & 0.421 & 0.415 & 0.54\% & -1.39\% \\ 

& sebert\_sat & 0.429 & 0.512 & 0.415 & 0.498 & 0.430 & 0.488 & -13.60\% & \multicolumn{1}{l|}{-9.24\%} & 0.396 & 0.489 & 0.382 & 0.433 & 0.379 & 0.426 & -11.77\% & -8.97\% \\ 

& sebert\_mul & 0.403 & 0.532 & 0.403 & 0.421 & 0.405 & 0.444 & -17.82\% & \multicolumn{1}{l|}{-15.57\%} & 0.427 & 0.500 & 0.383 & 0.419 & 0.387 & 0.451 & -8.83\% & -7.53\% \\
\hline





\end{tabular}

$\blacklozenge$ = Baseline for the BERT-based models, Variants of single task variants are suffixed as \_sat, whereas the multitask variants are suffixed as \_mul.\\
$\lozenge$=Legacy results using VSM without use of BERT models.
\end{table*}

==> tables/L2.tex <==
% \usepackage{multirow}

\begin{table*}[t!]
\centering
\caption{Performance of BERT-based models leveraging proposed architectures along with the baseline on L2 problem against two datasets - CM1 and Dronology}

% \jch{I feel like the improvements are a bit extreme because the baseline is quite terrible.  What if we renamed Baseline to ``Legacy'' and then used the Sat-BERT \& MSat\-BERT (bert\_sat) as the actual baseline for this work.  We compare that to legacy first and show significant improvement simply from using BERT*. After that, all comparisons are made against the HIGHER BAR baseline of the bert\_sat.  Alternately, and I think I like this plan better.  We first have legacy, then for each of the two major approaches we establish a NEW baseline (i.e., bert\_sat). We then compare the variants against that baseline, and finally we compare the SAT-*** vs. DSat\_BERT variants?}}
 \begin{subtable}[h]{\textwidth}
	    \centering
\begin{tabular}{c|c|c|cc|cc|cc|cc}\toprule \hline
L2                     &                    & \multicolumn{1}{c|}{Models} & \multicolumn{2}{c|}{100}                                      & \multicolumn{2}{c|}{300}                           & \multicolumn{2}{c|}{500}                                   & \multicolumn{2}{c}{Avg Improvement}                     \\ 
&                                        & &                       \multicolumn{1}{c}{F2}    & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{F2}      & \multicolumn{1}{c}{MAP}  \\ 
\hline
\multirow{17}{*}{CM-1}  

                       & \multirow{1}{*}{Legacy} & -               & 0.115                   & 0.199                    & 0.058                   & 0.167                    & 0.046                   & 0.166                     & \multicolumn{1}{c}{-}       & \multicolumn{1}{c}{-}\\ 
                       
                       
\hline 

                       & \multirow{6}{*}{Sat-BERT \& MSat-BERT} & bert\_sat             & 0.211                   & 0.264                    & 0.142                   & 0.189                    & 0.137                   & 0.164                    & 143.46\%                & 14.69\%                   \\ 

                       &                                         & bert\_mul             & 0.253                   & 0.346                    & 0.222                   & 0.263                    & 0.175                   & 0.208                    & 229.72\%                & 51.95\%                   \\ 

                       &                                         & scibert\_sat          & 0.225                   & 0.265                    & 0.270                   & 0.262                    & 0.269                   & 0.263                    & 318.01\%                & 49.32\%                   \\ 

                       &                                         & scibert\_mul          & 0.319                   & 0.338                    & 0.255                   & 0.274                    & 0.249                   & 0.253                    & 322.20\%                & 62.02\%                   \\ 

                       &                                         & sebert\_sat           & 0.318                   & 0.338                    & 0.207                   & 0.282                    & 0.231                   & 0.215                    & 280.80\%                & 55.87\%                   \\ 

                       &                                         & sebert\_mul           & 0.351                   & 0.388                    & 0.249                   & 0.322                    & 0.295                   & 0.367                    & 361.54\%                & 102.48\%                  \\ 

\cline{2-11}
   

                       & \multirow{6}{*}{DSat-BERT \& DMSat-BERT}  & bert\_sat             & 0.247                   & 0.303                    & 0.190                   & 0.192                    & 0.118                   & 0.112                    & 167.82\%                & 11.35\%                   \\ 

                       &                                         & bert\_mul             & 0.263                   & 0.339                    & 0.221                   & 0.261                    & 0.178                   & 0.205                    & 234.69\%                & 49.78\%                   \\ 

                       &                                         & scibert\_sat          & 0.286                   & 0.328                    & 0.223                   & 0.243                    & 0.237                   & 0.267                    & 285.55\%                & 56.90\%                   \\ 

                       &                                         & scibert\_mul          & 0.297                   & 0.377                    & 0.254                   & 0.295                    & 0.246                   & 0.251                    & 313.26\%                & 72.26\%                   \\ 

                       &                                         & sebert\_sat           & 0.280                   & 0.369                    & 0.250                   & 0.245                    & 0.190                   & 0.185                    & 264.66\%                & 47.85\%                   \\ 

                       &                                         & sebert\_mul           & 0.376                   & 0.397                    & 0.257                   & 0.286                    & 0.235                   & 0.256                    & 329.82\%                & 74.75\%                   \\
                       
% \usepackage{multirow}
\hline
\hline

\multirow{16}{*}{Dronology} 

% &                                         & Baseline              
                            & \multirow{1}{*}{Baseline} & -              & 0.114                   & 0.293                    & 0.042                   & 0.234                    & 0.028                   & 0.233             & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-}\\ 
                            
                            \cline{2-11}

                            & \multirow{6}{*}{Sat-BERT \& MSat-BERT} & bert\_sat             & 0.538                   & 0.678                    & 0.374                   & 0.488                    & 0.358                   & 0.439                    & 784.59\%                & 109.68\%                  \\ 
                            
                            &                                         & bert\_mul             & 0.469                   & 0.664                    & 0.462                   & 0.576                    & 0.395                   & 0.457                    & 878.42\%                & 123.15\%                  \\ 
                            
                            &                                         & scibert\_sat          & 0.534                   & 0.687                    & 0.435                   & 0.561                    & 0.450                   & 0.589                    & 942.93\%                & 142.53\%                  \\ 

                            &                                         & scibert\_mul          & 0.531                   & 0.731                    & 0.492                   & 0.636                    & 0.411                   & 0.542                    & 939.84\%                & 151.56\%                  \\ 

                            &                                         & sebert\_sat           & 0.633                   & 0.792                    & 0.498                   & 0.604                    & 0.491                   & 0.619                    & 1071.23\%               & 164.97\%                  \\ 

                            &                                         & sebert\_mul           & 0.603                   & 0.798                    & 0.499                   & 0.508                    & 0.458                   & 0.573                    & 1023.45\%               & 145.39\%                  \\ 

\cline{2-11}


                            & \multirow{6}{*}{DSat-BERT \& DMSat-BERT}  & bert\_sat             & 0.550                   & 0.710                    & 0.405                   & 0.562                    & 0.394                   & 0.490                    & 855.71\%                & 131.16\%                  \\ 

                            &                                         & bert\_mul             & 0.563                   & 0.705                    & 0.383                   & 0.463                    & 0.403                   & 0.482                    & 852.77\%                & 115.31\%                  \\ 

                            &                                         & scibert\_sat          & 0.510                   & 0.630                    & 0.471                   & 0.561                    & 0.339                   & 0.399                    & 829.50\%                & 108.90\%                  \\ 

                            &                                         & scibert\_mul          & 0.553                   & 0.724                    & 0.491                   & 0.600                    & 0.434                   & 0.488                    & 973.76\%                & 138.05\%                  \\ 

                            &                                         & sebert\_sat           & 0.532                   & 0.649                    & 0.491                   & 0.591                    & 0.506                   & 0.548                    & 1054.64\%               & 136.59\%                  \\ 

                            &                                         & sebert\_mul           & 0.597                   & 0.653                    & 0.527                   & 0.615                    & 0.504                   & 0.552                    & 1099.16\%               & 141.07\%                  \\

\hline
\end{tabular}
\end{subtable}
\end{table*}

==> tables/L2PLUS.tex <==
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\caption{Performance of BERT-based models leveraging proposed architectures along with the baseline on L2-PLUS problem against two datasets - CM1 and Dronology}
 \begin{subtable}[h]{\textwidth}
	    \centering
\begin{tabular}{c|c|c|cc|cc|cc|cc}\toprule \hline
L2-PLUS                    &                    & \multicolumn{1}{c|}{Models} & \multicolumn{2}{c|}{100}                                      & \multicolumn{2}{c|}{300}                           & \multicolumn{2}{c|}{500}                                   & \multicolumn{2}{c}{Avg Improvement}                     \\ 
&                                        & &                       \multicolumn{1}{c}{macro-F1}    & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{macro-F1} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{macro-F1} & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{macro-F1}      & \multicolumn{1}{c}{MAP}  \\ 
\hline


\multirow{14}{*}{CM-1}

                 & \multirow{1}{*}{Baseline} & -   & \multicolumn{1}{c}{-}        & 0.200                    & \multicolumn{1}{c}{-}        & 0.167                    & \multicolumn{1}{l}{-}        & 0.166                    & -               & \multicolumn{1}{c}{-}    \\ 
                       \cline{2-11}

                            & \multirow{6}{*}{Sat-BERT \& MSat-BERT} & bert\_sat    & 0.380                         & 0.334                    & 0.368                         & 0.167                    & 0.382                         & 0.164                    & -               & 21.78\%                   \\ 

                            &                                         & bert\_mul    & 0.402                         & 0.310                    & 0.346                         & 0.243                    & 0.358                         & 0.193                    & -               & 38.63\%                   \\ 

                            &                                         & scibert\_sat & 0.424                         & 0.365                    & 0.380                         & 0.200                    & 0.390                         & 0.238                    & -               & 48.35\%                   \\ 

                            &                                         & scibert\_mul & 0.397                         & 0.313                    & 0.356                         & 0.293                    & 0.357                         & 0.212                    & -               & 52.82\%                   \\ 

                            &                                         & sebert\_sat  & 0.369                         & 0.253                    & 0.380                         & 0.181                    & 0.387                         & 0.218                    & -               & 21.87\%                   \\ 

                            &                                         & sebert\_mul  & 0.412                         & 0.333                    & 0.380                         & 0.238                    & 0.370                         & 0.201                    & -               & 43.13\%                   \\ 

                            % &                                         &              & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}    &                 & \multicolumn{1}{l|}{}     \\ 
\cline{2-11}
                            & \multirow{6}{*}{DSat-BERT \& DMSat-BERT}  & bert\_sat    & 0.377                         & 0.295                    & 0.367                         & 0.193                    & 0.380                         & 0.152                    & -               & 17.93\%                   \\ 

                            &                                         & bert\_mul    & 0.399                         & 0.367                    & 0.355                         & 0.187                    & 0.345                         & 0.217                    & -               & 41.92\%                   \\ 

                            &                                         & scibert\_sat & 0.395                         & 0.286                    & 0.405                         & 0.237                    & 0.386                         & 0.187                    & -               & 32.18\%                   \\ 

                            &                                         & scibert\_mul & 0.403                         & 0.289                    & 0.355                         & 0.257                    & 0.352                         & 0.208                    & -               & 40.95\%                   \\ 

                            &                                         & sebert\_sat  & 0.367                         & 0.310                    & 0.394                         & 0.223                    & 0.388                         & 0.180                    & -               & 32.02\%                   \\ 

                            &                                         & sebert\_mul  & 0.400                         & 0.356                    & 0.375                         & 0.224                    & 0.371                         & 0.196                    & -               & 43.01\%                   \\ 
\hline
\hline

\multirow{14}{*}{Dronology} &                                         & Baseline     & \multicolumn{1}{l}{-}        & 0.270                    & \multicolumn{1}{l}{-}        & 0.254                    & \multicolumn{1}{l}{-}        & 0.233                    & -               & \multicolumn{1}{l}{-}    \\ 
\cline{2-11}
                            & \multirow{6}{*}{Sat-BERT \& MSat-BERT} & bert\_sat    & 0.466                         & 0.508                    & 0.431                         & 0.366                    & 0.432                         & 0.341                    & -               & 59.61\%                   \\ 

                            &                                         & bert\_mul    & 0.468                         & 0.501                    & 0.405                         & 0.408                    & 0.420                         & 0.403                    & -               & 73.20\%                   \\ 

                            &                                         & scibert\_sat & 0.450                         & 0.523                    & 0.442                         & 0.486                    & 0.463                         & 0.500                    & -               & 100.21\%                  \\ 

                            &                                         & scibert\_mul & 0.487                         & 0.606                    & 0.388                         & 0.488                    & 0.422                         & 0.454                    & -               & 104.06\%                  \\ 

                            &                                         & sebert\_sat  & 0.470                         & 0.569                    & 0.477                         & 0.408                    & 0.466                         & 0.402                    & -               & 81.56\%                   \\ 

                            &                                         & sebert\_mul  & 0.439                         & 0.550                    & 0.396                         & 0.420                    & 0.429                         & 0.421                    & -               & 83.41\%                   \\ 

                            % &                                         &              & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}    &                 & \multicolumn{1}{l|}{}     \\ 
\cline{2-11}
                            & \multirow{6}{*}{DSat-BERT \& DMSat-BERT}  & bert\_sat    & 0.483                         & 0.511                    & 0.440                         & 0.338                    & 0.420                         & 0.343                    & -               & 56.68\%                   \\ 

                            &                                         & bert\_mul    & 0.489                         & 0.518                    & 0.407                         & 0.411                    & 0.413                         & 0.372                    & -               & 71.34\%                   \\ 

                            &                                         & scibert\_sat & 0.482                         & 0.542                    & 0.477                         & 0.470                    & 0.463                         & 0.495                    & -               & 99.60\%                   \\ 

                            &                                         & scibert\_mul & 0.429                         & 0.565                    & 0.440                         & 0.456                    & 0.397                         & 0.403                    & -               & 87.35\%                   \\ 

                            &                                         & sebert\_sat  & 0.474                         & 0.505                    & 0.462                         & 0.394                    & 0.434                         & 0.417                    & -               & 73.86\%                   \\ 

                            &                                         & sebert\_mul  & 0.477                         & 0.522                    & 0.439                         & 0.367                    & 0.403                         & 0.430                    & -               & 74.15\%                   \\
\hline
\end{tabular}
\end{subtable}
\end{table*}

==> tables/L2PLUSUpdated.tex <==
\begin{table*}[t!]
\centering
\caption{Performance of BERT-based models leveraging the proposed architectures on L3 challenge against the two datasets - CM1 and Dronology.} 
 \begin{subtable}[h]{\textwidth}
	    \centering
\begin{tabular}{c|c|c|cc|cc|cc|cc}\toprule \hline
L2-PLUS                     &                    & \multicolumn{1}{c|}{Models} & \multicolumn{2}{c|}{100}                                      & \multicolumn{2}{c|}{300}                           & \multicolumn{2}{c|}{500}                                   & \multicolumn{2}{c}{Avg Improvement}                     \\ 
&                                        & &                       \multicolumn{1}{c}{macro\_F1}    & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{macro\_F1} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{macro\_F1} & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{macro\_F1}      & \multicolumn{1}{c}{MAP}  \\ 
\hline
\multirow{17}{*}{CM-1}

                        & \multirow{1}{*}{Legacy} & -               &-    & 0.200                   &-         & 0.167                    & -                   & 0.166                     & \multicolumn{1}{c}{-}       & \multicolumn{1}{c}{-}\\ 
\cline{2-11}

                            & \multirow{6}{*}{Sat-BERT \& MSat-BERT} & bert\_sat*   & 0.380                         & 0.334                    & 0.368                         & 0.167                    & 0.382                         & 0.164                    & -                                                         & 21.78\%                   \\ 
\cline{3-11}
                            &                                         & bert\_mul    & 0.402                         & 0.310                    & 0.346                         & 0.243                    & 0.358                         & 0.193                    & -                                                         & 18.62\%                   \\ 

                            &                                         & scibert\_sat & 0.424                         & 0.365                    & 0.380                         & 0.200                    & 0.390                         & 0.238                    & -                                                         & 24.71\%                   \\ 

                            &                                         & scibert\_mul & 0.397                         & 0.313                    & 0.356                         & 0.293                    & 0.357                         & 0.212                    & -                                                         & 32.68\%                   \\ 

                            &                                         & sebert\_sat  & 0.369                         & 0.253                    & 0.380                         & 0.181                    & 0.387                         & 0.218                    & -                                                         & 5.64\%                    \\ 
                            &                                         & sebert\_mul  & 0.412                         & 0.333                    & 0.380                         & 0.238                    & 0.370                         & 0.201                    & -                                                         & 21.58\%                   \\ 
\cline{2-11}

                            & \multirow{6}{*}{DSat-BERT \& DMSat-BERT}  & bert\_sat*   & 0.377                         & 0.295                    & 0.367                         & 0.193                    & 0.380                         & 0.152                    & -                                                         & 17.93\%                   \\ 
\cline{3-11}
                            &                                         & bert\_mul    & 0.399                         & 0.367                    & 0.355                         & 0.187                    & 0.345                         & 0.217                    & -                                                         & 21.49\%                   \\ 

                            &                                         & scibert\_sat & 0.395                         & 0.286                    & 0.405                         & 0.237                    & 0.386                         & 0.187                    & -                                                         & 14.23\%                   \\ 

                            &                                         & scibert\_mul & 0.403                         & 0.289                    & 0.355                         & 0.257                    & 0.352                         & 0.208                    & -                                                         & 22.72\%                   \\ 

                            &                                         & sebert\_sat  & 0.367                         & 0.310                    & 0.394                         & 0.223                    & 0.388                         & 0.180                    & -                                                         & 13.02\%                   \\ 

                            &                                         & sebert\_mul  & 0.400                         & 0.356                    & 0.375                         & 0.224                    & 0.371                         & 0.196                    & -                                                         & 21.82\%                   \\ 
\hline
\hline


\multirow{14}{*}{Dronology} 

                        & \multirow{1}{*}{Legacy} & -               &-    & 0.270                   &-         & 0.254                    & -                   & 0.233                     & \multicolumn{1}{c}{-}       & \multicolumn{1}{c}{-}\\ 
\cline{2-11}
                            & \multirow{6}{*}{Sat-BERT \& MSat-BERT} & bert\_sat*   & 0.466                         & 0.508                    & 0.431                         & 0.366                    & 0.432                         & 0.341                    & -                                                         & 59.61\%                   \\ 
\cline{3-11}
                            &                                         & bert\_mul    & 0.468                         & 0.501                    & 0.405                         & 0.408                    & 0.420                         & 0.403                    & -                                                         & 9.48\%                    \\ 

                            &                                         & scibert\_sat & 0.450                         & 0.523                    & 0.442                         & 0.486                    & 0.463                         & 0.500                    & -                                                         & 27.62\%                   \\ 

                            &                                         & scibert\_mul & 0.487                         & 0.606                    & 0.388                         & 0.488                    & 0.422                         & 0.454                    & -                                                         & 28.68\%                   \\ 

                            &                                         & sebert\_sat  & 0.470                         & 0.569                    & 0.477                         & 0.408                    & 0.466                         & 0.402                    & -                                                         & 13.90\%                   \\ 

                            &                                         & sebert\_mul  & 0.439                         & 0.550                    & 0.396                         & 0.420                    & 0.429                         & 0.421                    & -                                                         & 15.54\%                   \\ 
\cline{2-11}

                            & \multirow{6}{*}{DSat-BERT \& DMSat-BERT}  & bert\_sat*   & 0.483                         & 0.511                    & 0.440                         & 0.338                    & 0.420                         & 0.343                    & -                                                         & 56.68\%                   \\ 
\cline{3-11}
                            &                                         & bert\_mul    & 0.489                         & 0.518                    & 0.407                         & 0.411                    & 0.413                         & 0.372                    & -                                                         & 10.51\%                   \\ 

                            &                                         & scibert\_sat & 0.482                         & 0.542                    & 0.477                         & 0.470                    & 0.463                         & 0.495                    & -                                                         & 29.83\%                   \\ 

                            &                                         & scibert\_mul & 0.429                         & 0.565                    & 0.440                         & 0.456                    & 0.397                         & 0.403                    & -                                                         & 20.94\%                   \\ 

                            &                                         & sebert\_sat  & 0.474                         & 0.505                    & 0.462                         & 0.394                    & 0.434                         & 0.417                    & -                                                         & 12.32\%                   \\ 

                            &                                         & sebert\_mul  & 0.477                         & 0.522                    & 0.439                         & 0.367                    & 0.403                         & 0.430                    & -                                                         & 11.95\%                   \\
\hline
\end{tabular}
\end{subtable}
\vspace{5pt}\\
bert\_sat* = Baseline for the BERT-based models
\end{table*}

==> tables/L2baseline.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}

\begin{table}[!tb]
\centering
\caption{L2-Baseline -- two approaches -- Coverage Rate and Coverage Score}
\scalebox{0.7}{
\begin{tabular}{c|c|cc|cc|cc}\toprule \hline
L2                     &Samples                    & \multicolumn{2}{c|}{Coverage Rate} & \multicolumn{2}{c|}{Coverage Score}               &\multicolumn{2}{c}{MAX (L-Baseline)} \\ 
&         & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{F2}      & \multicolumn{1}{c}{MAP}  \\ 
\hline
                           
% ------------------------------------------
\multirow{3}{*}{CM1}       & 100                             & 0.111                   & 0.132                    & 0.115                   & 0.199                    & 0.115                   & 0.199                     \\ 

                           & 300                             & 0.051                   & 0.105                    & 0.058                   & 0.167                    & 0.058                   & 0.167                     \\ 

                           & 500                             & 0.041                   & 0.104                    & 0.046                   & 0.166                    & 0.046                   & 0.166                     \\ 

\hline
\multirow{3}{*}{Dronology} & 100                             & 0.106                   & 0.293                    & 0.114                   & 0.285                    & 0.114                   & 0.293                     \\ 

                           & 300                             & 0.041                   & 0.234                    & 0.042                   & 0.224                    & 0.042                   & 0.234                     \\ 

                           & 500                             & 0.026                   & 0.233                    & 0.028                   & 0.223                    & 0.028                   & 0.233                     \\


\hline
\end{tabular}}

\end{table}


==> tables/L2updated.tex <==
\input{tables/L2ModifiedTableLayout.tex}

\begin{table*}[t!]
\centering
\caption{\jch{See improved table layout in current Table \ref{tab:C1}.  Also I moved 'legacy' for all three datasets to a new SMALL table.  It just doesn't fit here very well.} Performance of BERT-based models leveraging the proposed architectures on L2 challenge against the two datasets - CM1 and Dronology. In this table, we report the performance gains for bert\_sat* over the Legacy Baseline - showing that the naive BERT model alone can significantly outperform the IR-based approaches. However, for the other variants, we consider bert\_sat* in each of the major approaches as our new baseline and report the average performance gain/loss.} 
% \jch{I feel like the improvements are a bit extreme because the baseline is quite terrible.  What if we renamed Baseline to ``Legacy'' and then used the Sat-BERT \& MSat\-BERT (bert\_sat) as the actual baseline for this work.  We compare that to legacy first and show significant improvement simply from using BERT*. After that, all comparisons are made against the HIGHER BAR baseline of the bert\_sat.  Alternately, and I think I like this plan better.  We first have legacy, then for each of the two major approaches we establish a NEW baseline (i.e., bert\_sat). We then compare the variants against that baseline, and finally we compare the SAT-*** vs. DSat\_BERT variants?}}
 \begin{subtable}[h]{\textwidth}
	    \centering
\begin{tabular}{c|c|c|cc|cc|cc|cc}\toprule \hline
L2                     &                    & \multicolumn{1}{c|}{Models} & \multicolumn{2}{c|}{100}                                      & \multicolumn{2}{c|}{300}                           & \multicolumn{2}{c|}{500}                                   & \multicolumn{2}{c}{Avg Improvement}                     \\ 
&                                        & &                       \multicolumn{1}{c}{F2}    & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP} & \multicolumn{1}{c}{F2} & \multicolumn{1}{c|}{MAP}         & \multicolumn{1}{c}{F2}      & \multicolumn{1}{c}{MAP}  \\ 
\hline
\multirow{17}{*}{CM-1}  

                       & \multirow{1}{*}{Legacy} & -               & 0.115                   & 0.199                    & 0.058                   & 0.167                    & 0.046                   & 0.166                     & \multicolumn{1}{c}{-}       & \multicolumn{1}{c}{-}\\ 
                       
                       \cline{2-11}

                            & \multirow{6}{*}{Sat-BERT \& MSat-BERT} & bert\_sat *           & 0.211                   & 0.264                    & 0.142                   & 0.189                    & 0.137                   & 0.164                    & 143.46\%                & 14.69\%                   \\ 

                            &                                         & bert\_mul             & 0.253                   & 0.346                    & 0.222                   & 0.263                    & 0.175                   & 0.208                    & 34.65\%                 & 32.34\%                   \\ 

                            &                                         & scibert\_sat          & 0.225                   & 0.265                    & 0.270                   & 0.262                    & 0.269                   & 0.263                    & 64.38\%                 & 33.26\%                   \\ 

                            &                                         & scibert\_mul          & 0.319                   & 0.338                    & 0.255                   & 0.274                    & 0.249                   & 0.253                    & 70.94\%                 & 42.62\%                   \\ 

                            &                                         & sebert\_sat           & 0.318                   & 0.338                    & 0.207                   & 0.282                    & 0.231                   & 0.215                    & 55.06\%                 & 36.18\%                   \\ 

                            &                                         & sebert\_mul           & 0.351                   & 0.388                    & 0.249                   & 0.322                    & 0.295                   & 0.367                    & 85.74\%                 & 80.33\%                   \\ 
\cline{2-11}

                            & \multirow{6}{*}{DSat-BERT \& DMSat-BERT}  & bert\_sat*            & 0.247                   & 0.303                    & 0.190                   & 0.192                    & 0.118                   & 0.112                    & 167.82\%                & 11.35\%                   \\ 

                            &                                         & bert\_mul             & 0.263                   & 0.339                    & 0.221                   & 0.261                    & 0.178                   & 0.205                    & 24.79\%                 & 43.79\%                   \\ 

                            &                                         & scibert\_sat          & 0.286                   & 0.328                    & 0.223                   & 0.243                    & 0.237                   & 0.267                    & 44.91\%                 & 58.07\%                   \\ 

                            &                                         & scibert\_mul          & 0.297                   & 0.377                    & 0.254                   & 0.295                    & 0.246                   & 0.251                    & 54.36\%                 & 67.81\%                   \\ 

                            &                                         & sebert\_sat           & 0.280                   & 0.369                    & 0.250                   & 0.245                    & 0.190                   & 0.185                    & 35.35\%                 & 38.58\%                   \\ 

                            &                                         & sebert\_mul           & 0.376                   & 0.397                    & 0.257                   & 0.286                    & 0.235                   & 0.256                    & 62.39\%                 & 69.77\%                   \\ 

\hline
\hline
\multirow{14}{*}{Dronology}

                       & \multirow{1}{*}{Legacy} & -               & 0.114                   & 0.293                    & 0.042                   & 0.234                    & 0.028                   & 0.233                    & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-}    \\  
                       
                       \cline{2-11}

                            & \multirow{6}{*}{Sat-BERT \& MSat-BERT} & bert\_sat*            & 0.538                   & 0.678                    & 0.374                   & 0.488                    & 0.358                   & 0.439                    & 784.59\%                & 109.68\%                  \\ 

                            &                                         & bert\_mul             & 0.469                   & 0.664                    & 0.462                   & 0.576                    & 0.395                   & 0.457                    & 6.98\%                  & 6.66\%                    \\ 

                            &                                         & scibert\_sat          & 0.534                   & 0.687                    & 0.435                   & 0.561                    & 0.450                   & 0.589                    & 13.78\%                 & 16.79\%                   \\ 

                            &                                         & scibert\_mul          & 0.531                   & 0.731                    & 0.492                   & 0.636                    & 0.411                   & 0.542                    & 15.04\%                 & 20.53\%                   \\ 

                            &                                         & sebert\_sat           & 0.633                   & 0.792                    & 0.498                   & 0.604                    & 0.491                   & 0.619                    & 29.39\%                 & 27.19\%                   \\ 

                            &                                         & sebert\_mul           & 0.603                   & 0.798                    & 0.499                   & 0.508                    & 0.458                   & 0.573                    & 24.53\%                 & 17.45\%                   \\ 
\cline{2-11}

                            & \multirow{6}{*}{DSat-BERT \& DMSat-BERT}  & bert\_sat*            & 0.550                   & 0.710                    & 0.405                   & 0.562                    & 0.394                   & 0.490                    & 855.71\%                & 131.16\%                  \\ 

                            &                                         & bert\_mul             & 0.563                   & 0.705                    & 0.383                   & 0.463                    & 0.403                   & 0.482                    & -0.29\%                 & -6.66\%                   \\ 

                            &                                         & scibert\_sat          & 0.510                   & 0.630                    & 0.471                   & 0.561                    & 0.339                   & 0.399                    & -1.67\%                 & -10.00\%                  \\ 

                            &                                         & scibert\_mul          & 0.553                   & 0.724                    & 0.491                   & 0.600                    & 0.434                   & 0.488                    & 10.73\%                 & 2.84\%                    \\ 

                            &                                         & sebert\_sat           & 0.532                   & 0.649                    & 0.491                   & 0.591                    & 0.506                   & 0.548                    & 15.54\%                 & 2.77\%                    \\ 

                            &                                         & sebert\_mul           & 0.597                   & 0.653                    & 0.527                   & 0.615                    & 0.504                   & 0.552                    & 22.25\%                 & 4.67\%                    \\
\hline

\hline
\end{tabular}
\end{subtable}
\vspace{5pt}\\
bert\_sat* = Baseline for the BERT-based models, Variants of single task variants are suffixed as \_sat, whereas the multitask variants are suffixed as \_mul.
\end{table*}

==> test-Approach.tex <==
\section{Approach}
\label{sec:Approach}

Effective RSA bridges the semantic gap between the requirement and the set of design elements that have been linked to it.  We hypothesize that this type of semantic analysis would benefit from the use of Pretrained Language Models such as BERT. Therefore we discuss the fundamentals ofthe BERT architecture, and provide a detailed description of the four models we we applied to the RSA problem. The selected models include Sat-BERT, MSat-BERT, DSat-BERT, and DMSat-BERT.

\subsection{Language Models and BERT}
Language models are designed to predict next elements of a sequence. In particular, given a sentence with a sequence of words \{w$_1$, w$_2$, ..., w$_k$\}, Language Models (LMs) calculate the probability of either the next word in the sequence i.e. P(w$_k$ $\mid$ $w_{1:k-1}$) or the probability of the whole sequence i.e. P(w$_{1:k}$). Therefore LMs are generally described as the probability distribution over a sequence of words\cite{jurafskyspeech}.

Transformers are attention-based mechanisms \cite{vaswani2017attention} that have substantially improved a number of diverse natural language processing (NLP) tasks. As a result, there have been a plethora of studies using transformers. To that end, Devlin et al. \cite{devlin2018bert} proposed an encoder-based language representation model called Bidirectional Encoders Representations from Transformers, widely known as BERT. BERT is trained on two tasks. The first is Masked Language Modeling (MLM) in which word(s) are randomly masked and the BERT is trained to replace them with the same words, and the second is Next Sentence Prediction (NSP) in which BERT is trained to understand dependencies across sentences thereby alleviating the problem of unidirectionality.

BERT is trained using the pretrain-fine paradigm whichconsists of a pretraining and fine-tuning stage. In the pretraining stage, the BERT-based model is fed with a huge corpus of data, and then fine-tuned using labeled data related to the targeted downstream tasks. To create a unified architecture for performing different tasks, BERT can be fine-tuned by adding an additional output layer commonly referred to as the \textbf{task head} \cite{devlin2018bert}.

\subsection{BERT for Requirements Satisfaction Assessment}
For purposes of automating the RSA problem we explore four different BERT architectures i.e. Sat-BERT, DSat-BERT, MSat-BERT, MDSat-BERT for RSA. In this naming scheme, `Sat' stands for Requirements SATisfaction analysis, and therefore Sat-BERT and DSat-BERT are vanilla solutions using single and dual architectures applied to the RSA problem. In contrast, MSat-BERT and MDSat-BERT are extensions that incorporate multi-tasking. For each of these architectures we experiment with three general purpose language models - BERT \cite{devlin2018bert}, scibert \cite{beltagy2019scibert} and sebert \cite{lin2022enhancing}. These models share the same underlying principles;  however, they have been trained using different training data to support domain-specific tasks. BERT is trained on a general corpus of data i.e. Wikipedia and BookCorpus \cite{zhu2015aligning}, while scibert is trained on a large multi-domain corpus of scientific publications, and sebert on a general software engineering domain obtained from millions of OSS projects on GitHub.

In the following sub-sections, we discuss the architectures in details.



\begin{figure}[h]
  \begin{center}
    \includegraphics[width=.3\columnwidth]{images/SAT-BERT.PNG}
  \end{center}
  \caption{Sat-BERT}
  \label{fig:satBERT}
\end{figure}


\begin{figure}[h]
  \begin{center}
  %JCH: THere 
  \includegraphics[width=.5\columnwidth]{images/MSAT-BERT.PNG}
    % \includegraphics[width=2.8in, height=1.8in]{images/MSAT-BERT.PNG}
  \end{center}
  \caption{MSat-BERT}
  \label{fig:msatBERT}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=.5\columnwidth]{images/DUAL-BERT.PNG}
  \end{center}
  \caption{DSat-BERT}
  \label{fig:dsatBERT}
\end{figure}


\subsubsection{\textbf{Sat-BERT}}

As depicted in Fig \ref{fig:satBERT}, Sat\_BERTis utilizes one BERT model to encode inputs as follows. First,  all the design elements linked to a corresponding requirement are concatenated with the requirement they are linked to as follows. First the tokens of the design elements $D_1$ \& $D_2$ are concatenated with a special token [SEP] between each element. Then the resulting string is concatenated concatenated to the requirement tokens forming a single sequence $I_{sat}$ s.t. $I_{sat}$ = $[CLS]$ \textit{$r_1$, $r_2$, ..., $r_N$} $[SEP]$ \textit{$d_{1,1}$, $d_{1,2}$, ..., $d_{1,N}$} $[SEP]$ \textit{$d_{2,1}$, $d_{2,2}$, ..., $d_{2,N}$} $[SEP]$, where $[CLS]$ and $[SEP]$ are special tokens marking the start and the end of the sentences respectively. 



The transformed representation of the requirement-design pair i.e. $I_{sat}$  is then fed to the BERT model, which generates a hidden matrix of 768 dimensions (default for BERT). The hidden matrix is passed through the series of feed-forward neural networks, which compresses the matrix into a lower dimension. Finally, a classification head categorizes the input into the specified number of classes by assigning the probabilities calculated using the Softmax function to produce a probability distribution. 
% I moved this to earlier at the point at which people can remember what C1, C2, and C3 actually are.
%While challenges C1 and C2, as discussed in Section II are binary classification problem with two probable outcomes i.e. satisfied or unsatisfied, C3 is a multi-class classification problem with three probable outputs i.e. satisfied, corrupt, or incomplete (missing). \vspace{5pt}



\subsubsection{\textbf{MSat-BERT}}
MSat-BERT is an extension to the Sat-BERT, in which the auxiliary task of link prediction is added by including an extra classification head in the single BERT model as shown in Fig \ref{fig:msatBERT}. The use of auxiliary tasks introduces multitask learning. The rationale for utilizing multitasking for finetuning a model is based on the way humans learn. Intuitively, humans first learn to solve easy problems, and then use the knowledge they have acquired to solve progressively more complex problem\cite{ruder2017overview}. 
%presented a more compelling example as to how the humans master new skills through excelling in simpler but related task using the movie \textit{'The Karate Kid'} as a reference.
Caruana et al., \cite{caruana1997multitask} described the use of related skills formaster a main task as an inductive transfer mechanism, and demonstrated better generalization across various tasks using Multitask Learning (MTL). They argued that many aspects of rich information sources are not leveraged in single-task Learning, whereas MTL, utilizes the information contained in training signals from different tasks as long as they are drawn from the same domain. \jch{If you are going to tell us that hard- and soft-parameter learning exist, then you should at least summarize them and tell us which you used and WHY it was selected.} There are two different ways to perform MTL, referred to as hard-parameter and soft-parameter sharing \cite{ruder2017overview}. 


% In this study, we propose two MTL-based architectures, namely MSat-BERT, and DMSat-BERT. -- removing the DMSat
We adopt the most commonly used approach i.e. hard-parameter sharing \cite{caruana1993multitask} which involves sharing the hidden layers among various tasks, while having distinct task-specific layers. Therefore, each of our two tasks,  i.e. satisfaction prediction \textit{(main)} and trace link prediction \textit{(auxiliary)} are assigned their own layers. Our experimental results show that in most cases, MTL outperforms the basic BERT artchitectures. \vspace{5pt}



%     \vspace{5pt}
\textbf{MSat-BERT} follows the same transformation as Sat-BERT for the main task i.e. satisfaction prediction; however, for the link prediction, \jch{instead of concatenating all design elements to the requirement they are linked to, we perform a pairwise combination of each requirement to each of its design elements s.t.} $I_{link}$ = \{$[CLS]$ \textit{$r_1$, $r_2$, ..., $r_N$} $[SEP]$ \textit{$d_{1,1}$, $d_{1,2}$, ..., $d_{1,N}$} $[SEP]$, $[CLS]$ \textit{$r_1$, $r_2$, ..., $r_N$} $[SEP]$ \textit{$d_{2,1}$, $d_{2,2}$, ..., $d_{2,N}$} $[SEP]$\}. After the transformation, the shared BERT model is fed with both $I_{sat}$ and $I_{link}$ which outputs two respective hidden state matrices. The matrices are then passed to their respective task-specific classification head, and the individual losses are obtained via Cross Entropy loss. Mathematically, 

If $L_{sat}$ \& $L_{link}$ are the two losses for satisfaction and link prediction tasks respectively, we minimize the multitask objective as:
\begin{equation}
    \begin{aligned}
    L = L_{sat} + \lambda L_{link} \\
    \end{aligned}
    \label{eq:multiloss}
\end{equation}

where $L_{sat}$, and $L_{link}$ are obtained via Cross Entropy (CE) Loss over their size of their respective training data. Mathematically,
        
\begin{equation}
        CE = -\sum_{n=1}^{output size} yi.log\hat{yi}
        \label{eq:CE}
\end{equation}
% \jch{See how I created a label in the above equation? You need to do it and then reference all equations using their labels e.g., \ref{eq:CE}.  Please fix all hard-coded figures, tables, equations. We can't hard-code!}

% \ap{sure}

\jch{In equation \ref{eq:multiloss}}, we assign higher value of importance to the satisfaction task as compared to the auxiliary link prediction task. We set the value of $\lambda $ to 0.5 for minimizing the multitask objectives in all the MTL related experiments.\\



\subsubsection{\textbf{DSat-BERT}}


\ap{Jane, this is different from the DMSat, this is just the dual version -- this still might need edit. I think I confused you keeping the comment just below this.}

As shown in Fig 3, DSat-BERT architecture makes use of the two BERT models. In this proposed architecture, one of the BERT models say M1 is fed with unaltered natural language requirements and design elements, whereas the other say M2 is served with requirement and design chunks. Chunks are simply the breakdown of natural language text into smaller fragments with some predefined grammar, which we discuss on details in Section IV. We believe that providing one of the models with knowledge relating only to chunks while providing the other with complete natural language will help in better generalization as the models can pay more attention to the important concepts. 

DSat-BERT implements the similar transformation technique as that of Sat-BERT. While the maximum sequence length for the model M1 is set to the default size of 512, we shrink the M2's maximum sequence length to 128, as chunks are refined and are shorter in length. The outputs from the models M1 and M2 of size 512*768 and 128*768 respectively are then concatenated to form a hidden representation of the size 740*768. The concatenated matrix then goes through the same steps as that of Sat-BERT. \\

% \end{itemize}
    % \ap{I think we can get rid of DMSat as it doesn't necessarily provide any improvements to the other models. Also we don't report the results from this experiment as it doesn't make an impact more or less}

    \jch{That's fine.  Please remove it throughout the paper. Actually, if I understood it correctly, I don't think it necessarily makes sense because it seems to focus on links (i.e., R to D pairwise concatenations and probably doesn't give enough information about the groups??}
    
    % \ap{yes, and since the dual architecture didn't perform as good as the single architecture, I think introducing multi-tasking to dual architecture doesn't really help. Also the performance degrades due to negative transfer as we see with MSat-BERT for C3 cases.}
    
% \subsubsection{\textbf{DMSat-BERT}}
%Not editing if it is going!
% Similar to the DSat-BERT architecutre, DMSat-BERT also makes use of the two BERT encoders as shown in Fig 4. Fed with the same inputs i.e. the complete natural language to the one model and chunks to another, the only difference between the two architectures is the introduction of MTL on DMSat-BERT. We add an extra link prediction task that branches out of the model processing the complete natural language, while the other architecture of the model remains the same as that of DSat-BERT. 
